Empowering Social Service with AI: Insights from a Participatory Design Study with Practitioners

In social service, administrative burdens and decision-making challenges often hinder practitioners from performing effective casework. Generative AI (GenAI) offers significant potential to streamline these tasks, yet exacerbates concerns about overreliance, algorithmic bias, and loss of identity within the profession. We explore these issues through a two-stage participatory design study. We conducted formative co-design workshops (\textit{n=27}) to create a prototype GenAI tool, followed by contextual inquiry sessions with practitioners (\textit{n=24}) using the tool with real case data. We reveal opportunities for AI integration in documentation, assessment, and worker supervision, while highlighting risks related to GenAI limitations, skill retention, and client safety. Drawing comparisons with GenAI tools in other fields, we discuss design and usage guidelines for such tools in social service practice.

==> sections-old/0_abstract.tex <==
\begin{abstract}
\begin{abstract}
% Social service practitioners face multiple obstacles in their work, including administrative burdens and challenges in decision-making. Generative AI has the potential to streamline these tasks and improve client outcomes. However, these systems exacerbate existing concerns about AI such as overreliance, erosion of worker skill, and algorithmic bias, and risk undermining the professional discretion essential to social service workers. In this paper, we explore these issues through a participatory design study with 51 social service practitioners. We present an empirical investigation into the interaction between practitioners and a co-designed prototype AI tool, which assists in client assessment and intervention planning. Through thematic analysis, we propose a framework describing the interplay between the core ethos of practitioners, practitioner attitudes towards AI, and the resulting considerations for designing AI systems. We also propose a framework for generative AI in human-AI collaboration, and conclude with novel design guidelines for AI systems in the sector.

In social service, administrative burdens and decision-making challenges hinder practitioners from performing effective casework. Generative AI can potentially streamline or automate these tasks, but also exacerbates existing concerns about AI such as overreliance, algorithmic bias, and loss of identity within the profession. We explore these issues through a participatory design study \textit{(n=51)}, investigating the interactions between practitioners and a co-designed AI tool for client assessment and intervention planning. We discover novel use cases for AI in this sector, and discuss how the interplay between the core ethos of practitioners, their attitudes towards AI, and the resulting considerations for the effective design of such systems. We propose an alternative framing of AI in the context of human-AI collaboration, and conclude with new design guidelines for AI systems in the social service sector.
% and algorithmic bias, and risks replacing the professional discretion at the heart of social work and threatening the profession itself. 


\end{abstract}

==> sections-old/1_introduction.tex <==
\section{Introduction}

The social service sector is crucial for a just and humane society, addressing various social injustices and supporting the well-being of individuals and communities \cite{difranks2008social}. Social service agencies render critical services such as client home visits, case analysis, and intervention planning, aiming to aid vulnerable clients in the best way possible. Social service practitioners (SSPs) must consider the myriad interacting factors in clients' social networks, physical environment, and intrapersonal cognitive and emotional systems, in context of clients' beliefs, perceptions, and desires, and all while respecting individual worth and dignity \cite{rooney2017direct}. This requires extensive training and hands-on experience, which may be challenging given the endlessly varying situations a worker may encounter \cite{rooney2017direct}.
% social work is hard -> needs experiences

These demands put a strain on the limited pool of social service manpower \cite{cho2017determinants}. SSPs grapple with time-consuming data processing \cite{singer_ai_2023, tiah_can_2024} and administrative \cite{meilvang_working_2023} tasks, compounded by the psychologically stressful nature of the job \cite{kalliath2012work}. Newer workers may experience challenging, unfamiliar client interactions, while experienced workers also face the added burden of mentoring junior workers. Current artificial intelligence (AI) systems aim to alleviate this through \textit{decision-support tools} \cite{gambrill2001need, de2020case, brown2019toward} which provide statistically validated assessments of client conditions \cite{gillingham2019can, van2017predicting}, thereby raising service quality and consistency. However, attempts to integrate AI systems in social service have faced a myriad of difficulties: mistrust in and uncertainty about technology \cite{gambrill2001need, brown2019toward}, worker confusion due to unclear organisational direction \cite{kawakami2022improving}, AI systems' inability to include local and contextual knowledge, and fear of AI potentially replacing jobs. As such, many attempts have been met with failure and inadequacies \cite{saxena2021framework, kawakami2022improving}.

% Recent, more promising systems powered by Large Language Models (LLMs) \cite{socialworkmagic2024, caseworthy2024} provide more flexible and detailed analyzes and recommendations to clients. Their ability to efficiently process vast amount of heterogeneous case data and provide a wide range of useful outputs to users significantly increases their utility to SSPs.

% MH: social work is hard -> manpower is not enough -> ai can help human judgment to lighten workload -> llm is better
% i feel a bit disconnected when i read new workers and experienced workers, why this message is important? i know that we will talk about the supervision stuffs in results, but the motivation seems can be strengthened? Like manpower is not enough is because new -> experienced is not easy..?

% MH: why talked about human judgment here? deciding the intervention protocol mentioned in the first paragraph? i feel decide intervention scheme and provide care need to be aligned? like 'provide the consistent, high-quality, and personalized care' = manpower, but 'Deciding how to help a given client is an intricate task' = manpower? i guess this can be clarified clearer. I feel manpower = labor, but decision-making is not very similar with this word
% \cite{socialworkmagic2024, caseworthy2024} they are LLM system for social work already? or just LLMs? how about change their position here 'These systems hold vast potential in significantly advancing the state of the social service sector \cite{socialworkmagic2024, caseworthy2024}.'

% Digital systems have long served to alleviate some of the burden, by both deputising for workers in client-facing care \cite{ruggiano2023examining, li2023systematic} 


Recent technological advancements, in particular generative AI, have the potential to play a greater, transformative role in the social service sector. Generative AI systems are capable of a wider range of tasks, including analysing written case recordings, performing qualitative risk assessments, providing crisis assistance, and aiding prevention efforts \cite{reamer_artificial_2023}.  
% which can generate novel outputs ranging from text reports to case assessments from large amounts of training data, are qualitatively different from most historical examples of automation technologies \cite{noy2023experimental}, and offer significant potential to transform the social service sector, with its ability to handle a myriad of social service tasks like analyzing case data, performing risk assessments, provide crisis assistance and prevention efforts, enhance social service outcomes and more \cite{reamer_artificial_2023}. This is especially crucial in a time-pressed sector like social service that suffers from resource constraints and highly manual processes, thereby helping to reduce the burdens faced by SSPs and freeing up their time to better serve clients, organizations and communities \cite{tiah_can_2024, fernando_integration_2023}. These systems hold vast potential in significantly advancing the state of the social service sector. Generative AI  
However, despite their advantages, these systems may exacerbate existing concerns with AI, risk overreliance \cite{van2023chatgpt} and potentially erode the human skills and values \cite{littlechild2008child, oak2016minority} core to the social service profession. 
% \cite{kawakami2022improving, de2020case} and adjacent healthcare \cite{devaraj2014barriers, elwyn2013many} sectors investigates systems that are vastly more primitive and limited in scope. 
As a novel technology, the efficacy of generative AI systems are still largely under-explored and untested in extant research \cite{gambrill2001need, de2020case, brown2019toward}, thus necessitating deeper scrutiny of AI technologies in social service. 

% Such systems, however, pale in comparison to the opportunities afforded by recent Large Language Models (LLMs), which demonstrate excellent performance in aggregating, understanding, and analysing large amounts of information. This lends them the ability to decision-making assistants in complex use cases. The core of social work is in humanising and thoroughly analysing each client,  The social work field offers many instances where information about a client must be organised, analysed, and weighed, in order to come up with a suitable and tailored intervention plan. This task is highly complex, since information can be missed or misinterpreted and theories can be wrongly applied by fallible humans. Modern LLMs like GPT-4 \cite{achiam2023gpt} seem well-placed to reduce human error and workload, with their ability to process large quantities of information almost instantly. 

% Uniquely, social work also presents the concern of responsibility attribution. Unlike, say, a travel planner that recommends holiday destinations or an ecommerce algorithm that suggests products, a social work assistant tool produces outputs with weighty moral implications. As a case worker's recommendations to and therapeutic work with a client can significantly affect their life trajectory, adopting an AI's suggestions leads to the natural question of who should be blamed for unfavourable outcomes. Blindly following AI guidance is clearly inappropriate. The resulting questions are therefore the degree to which AI guidance should be followed, and how AI tools should be designed and implemented to provide the right amount of guidance.

% These questions cannot be answered solely by system designers. The insight of users, i.e. social work practitioners, is invaluable in effective co-design of social work assistant tools.

% To fully investigate the risks, unknowns, and opportunities in AI-powered social service systems, 
To address this gap, this study therefore co-designs and pilots a novel generative AI tool with 51 SSPs, to better understand practitioners' perspectives on implementing AI in the social service sector. Uniquely, our study includes a diverse range of roles spanning the full range of social service practice, including many caseworkers who serve the general population, thus offering a broader perspective than past studies with more specialised caseworkers.
% we conduct a participatory design (PD) study to integrate the unique expertise and perspectives of SSPs with traditional computer system design. We conduct the study in two stages. 
We first run preliminary workshops with 27 SSPs to examine the place of AI within social service. From the insights gathered, we then build a prototype AI tool and conduct user testing and focus group discussions (FGDs) with 24 additional SSPs. Through thematic analysis of practitioners' responses, we develop a framework synthesising the critical values and attitudes of SSPs towards AI use. Finally, we present a set of guidelines for the effective conceptualisation and development of AI tools. 

% MH: I guess need to say why voice from social work practitioners is important can be elaborated, in the previous paragraph
% so here I still didn't get why mention new and experienced at first? I feel we may need at least one sentence here to echo

Overall, our study offers an empirically-grounded understanding of how workers use and perceive AI, shedding new light on the challenges and opportunities of generative AI in the social service sector and beyond. This paper makes the following contributions:
\begin{itemize}
    \item We conduct an empirical study to uncover new ways AI can complement social service practice;
    \item We develop a framework for understanding the role and place of AI in the social service sector;
    \item We propose a framework for designers that extends the use of AI \textit{beyond decision support} to inform the design of future AI tools in social service and broader sectors.
\end{itemize}

% This paper makes the following contributions:
% \begin{itemize}
%     \item We conduct empirical studies on the opportunities and requirements of AI tools in the social sector;
%     \item We develop a foundational framework for understanding the role and place of AI in the social service sector;
%     \item We develop a foundational framework for approaching the design of modern AI tools for social service and related sectors.
% \end{itemize}

==> sections-old/2_relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}

\subsection{Current AI Tools for Social Service}
\label{subsec:relatedtools}
% the title I feel is quite broad

Harnessing technology for social good has always been a grand challenge in social service \cite{berzin_practice_2015}. As early as the 90s, artificial neural networks and predictive models have been employed as tools for risk assessments, decision-making, and workload management in sectors like child protective services and mental health treatment \cite{fluke_artificial_1989, patterson_application_1999}. The recent rise of generative AI is poised to further advance social service practice, facilitating the automation of administrative tasks, streamlining of paperwork and documentation, optimisation of resource allocation, data analysis, and enhancing client support and interventions \cite{fernando_integration_2023, perron_generative_2023}.

Today, AI solutions are increasingly being deployed in both policy and practice \cite{goldkind_social_2021, hodgson_problematising_2022}. In clinical social work, AI has been used for risk assessments, crisis management, public health initiatives, and education and training for practitioners \cite{asakura_call_2020, gillingham2019can, jacobi_functions_2023, liedgren_use_2016, molala_social_2023, rice_piloting_2018, tambe_artificial_2018}. AI has also been employed for mental health support and therapeutic interventions, with conversational agents serving as on-demand virtual counsellors to provide clinical care and support \cite{lisetti_i_2013, reamer_artificial_2023}.
% commercial solutions include Woebot, which simulates therapeutic conversation, and Wysa, an “emotionally intelligent” AI coach, powered by evidenced-based clinical techniques \cite{reamer_artificial_2023}. 
% Non-clinical AI agents like Replika and companion robots can also provide social support and reduce loneliness amongst individuals \cite{ahmed_humanrobot_2024, chaturvedi_social_2023, pani_can_2024, ta_user_2020}.

Present research largely focuses on \textit{\textbf{AI-based decision support tools}} in social service \cite{james_algorithmic_2023, kawakami2022improving}, especially predictive risk models (PRMs) used to predict social service risks and outcomes \cite{gillingham2019can, van2017predicting}, like the Allegheny Family Screening Tool (AFST), which assesses child abuse risk using data from US public systems \cite{chouldechova_case_2018, vaithianathan2017developing}. Elsewhere, researchers have also piloted PRMs to predict social service needs for the homeless using Medicaid data\cite{erickson_automatic_2018, pourat_easy_2023}, and AI-powered algorithms to promote health interventions for at-risk populations, such as HIV testing among Californian homeless \cite{rice_piloting_2018, yadav_maximizing_2017}.

\subsection{Generative AI and Human-AI Collaboration}
\label{subsec:relatedworkhaicollaboration}
Beyond decision-making algorithms and PRMs, advancements in generative AI, such as large language models (LLMs), open new possibilities for human-AI (HAI) collaboration in social services. 
LLMs have been called "revolutionary" \cite{fui2023generative} and a "seismic shift" \cite{cooper2023examining}, offering "content support" \cite{memmert2023towards} by generating realistic and coherent responses to user inputs \cite{cascella2023evaluating}. Their vastly improved capabilities and ubiquity \cite{cooper2023examining} makes them poised to revolutionise work patterns \cite{fui2023generative}. Generative AI is already used in fields like design, writing, music, \cite{han2024teams, suh2021ai, verheijden2023collaborative, dhillon2024shaping, gero2023social} healthcare, and clinical settings \cite{zhang2023generative, yu2023leveraging, biswas2024intelligent}, with promising results. However, the social service sector has been slower in adopting AI \cite{diez2023artificial, kawakami2023training}.

% Yet, the social service sector is one that could perhaps stand to gain the most from AI technologies. As Goldkind \cite{goldkind_social_2021} writes, social service, as a "values-centred profession with a robust code of ethics" (p. 372), is uniquely placed to inform the development of thoughtful algorithmic policy and practice. 
Social service, however, stands to benefit immensely from generative AI. SSPs work in time-poor environments \cite{tiah_can_2024}, often overwhelmed with tedious administrative work \cite{meilvang_working_2023} and large amounts of paperwork and data processing \cite{singer_ai_2023, tiah_can_2024}. 
% As such, workers often work in time-poor environments and are burdened with information overload and administrative tasks \cite{tiah_can_2024, meilvang_working_2023}. 
Generative AI is well-placed to streamline and automate tasks like formatting case notes, formulating treatment plans and writing progress reports, which can free up valuable time for more meaningful work like client engagement and enhance service quality \cite{fernando_integration_2023, perron_generative_2023, tiah_can_2024, thesocialworkaimentor_ai_nodate}. 

Given the immense potential, there has been emerging research interest in HAI collaboration and teamwork in the Human-Computer Interaction and Computer Supported Cooperative Work space \cite{wang_human-human_2020}. HAI collaboration and interaction has been postulated by researchers to contribute to new forms of HAI symbiosis and augmented intelligence, where algorithmic and human agents work in tandem with one another to perform tasks better than they could accomplish alone by augmenting each other's strengths and capabilities  \cite{dave_augmented_2023, jarrahi_artificial_2018}.

However, compared to the focus on AI decision-making and PRM tools, there is scant research on generative AI and HAI collaboration in the social service sector \cite{wykman_artificial_2023}. This study therefore seeks to fill this critical gap by exploring how SSPs use and interact with a novel generative AI tool, helping to expand our understanding of the new opportunities that HAI collaboration can bring to the social service sector.

\subsection{Challenges in AI Use in Social Service}
\label{subsec:relatedworkaiuse}

% Despite the immense potential of AI systems to augment social work practice, there are multiple challenges with integrating such systems into real-life practice. 
Despite its evident benefits, multiple challenges plague the integration of AI and its vast potential into real-life social service practice.
% Numerous studies have investigated the use of PRMs to help practitioners decide on a course of action for their clients. 
When employing algorithmic decision-making systems, practitioners often experience tension in weighing AI suggestions against their own judgement \cite{kawakami2022improving, saxena2021framework}, being uncertain of how far they should rely on the machine. 
% Despite often being instructed to use the tool as part of evaluating a client, 
Workers are often reluctant to fully embrace AI assessments due to its inability to adequately account for the full context of a case \cite{kawakami2022improving, gambrill2001need}, and lack of clarity and transparency on AI systems and limitations \cite{kawakami2022improving}. Brown et al. \cite{brown2019toward} conducted workshops using hypothetical algorithmic tools 
% to understand service providers' comfort levels with using such tools in their work,
and found similar issues with mistrust and perceived unreliability. Furthermore, introducing AI tools can  create new problems of its own, causing confusion and distrust amongst workers \cite{kawakami2022improving}. Such factors are critical barriers to the acceptance and effective use of AI in the sector.

\citeauthor{meilvang_working_2023} (2023) cites the concept of \textit{boundary work}, which explores the delineation between "monotonous" administrative labour and "professional", "knowledge based" work drawing on core competencies of SSPs. While computers have long been used for bureaucratic tasks like client registration, the introduction of decision support systems like PRMs stirred debate over AI "threatening professional discretion and, as such, the profession itself" \cite{meilvang_working_2023}. Such latent concerns arguably drive the resistance to technology adoption described above. Generative AI is only set to further push this boundary, 
% these concerns are only set to grow in tandem with the vast capabilities of generative and other modern AI systems. Compared to the relatively primitive AI systems in past years, perceived as statistical algorithms \cite{brown2019toward} turning preset inputs like client age and behavioural symptoms \cite{vaithianathan2017developing} into simple numerical outputs indicating various risk scores, modern AI systems are vastly more capable: LLMs 
with its ability to formulate detailed reports and assessments that encroach upon the "core" work of SSPs.
% accept unrestricted and unstructured inputs and return a range of verbose and detailed evaluations according to the user's instructions. 
Introducing these systems exacerbate previously-raised issues such as understanding the limitations and possibilities of AI systems \cite{kawakami2022improving} and risk of overreliance on AI \cite{van2023chatgpt}, and requires a re-examination of where users fall on the algorithmic aversion-bias scale \cite{brown2019toward} and how they detect and react to algorithmic failings \cite{de2020case}. We address these critical issues through an empirical, on-the-ground study that to our knowledge is the first of its kind since the new wave of generative AI.

% W 

% Yet, to date, we have limited knowledge on the real-world impacts and implications of human-AI collaboration, and few studies have investigated practitioners’ experiences working with and using such AI systems in practice, especially within the social work context \cite{kawakami2022improving}. A small number of studies have explored practitioner perspectives on the use of AI in social work, including Kawakami et al. \cite{kawakami2022improving}, who interviewed social workers on their experiences using the AFST; Stapleton et al. \cite{stapleton_imagining_2022}, who conducted design workshops with caseworkers on the use of PRMs in child welfare; and Wassal et al. \cite{wassal_reimagining_2024}, who interviewed UK social work professionals on the use of AI. A common thread from all these studies was a general disregard for the context and users, with many practitioners criticising the failure of past AI tools arising from the lack of participation and involvement of social workers and actual users of such systems in the design and development of algorithmic systems \cite{wassal_reimagining_2024}. Similarly, in a scoping review done on decision-support algorithms in social work, Jacobi \& Christensen \cite{jacobi_functions_2023} reported that the majority of studies reveal limited bottom-up involvement and interaction between social workers, researchers and developers, and that algorithms were rarely developed with consideration of the perspective of social workers.
% so the \cite{yang_unremarkable_2019} and \cite{holten_moller_shifting_2020} are not real-world impacts? real-world means to hear practitioner's voice? I feel this is quite important but i didnt get this point in intro!

% why mentioning 'which have largely focused on existing ADS tools (e.g., AFST)'? i can see our strength is more localized, but without basic knowledge of social work i didnt get what's the 'departure' here orz
% the paragraph is great! do we need to also add one in line 20 21?

\subsection{Designing AI for Social Service through Participatory Design}
\label{subsec:relatedworkpd}
% i think it's important! but maybe not a whole subsection? but i feel the strong connection with practitioners is indeed one of our novelties and need to highlight it, also in intro maybe
% Participatory design (PD) has long been used extensively in HCI \cite{muller1993participatory}, to both design effective solutions for a specific community and gain a deep understanding of that community. Of particular interest here is the rich body of literature on PD in the field of healthcare \cite{donetto2015experience}, which in this regard shares many similarities and concerns with social work. PD has created effective health improvement apps \cite{ryu2017impact}, 

% PD offers researchers the chance to gather detailed user requirements \cite{ryu2017impact}...

Participatory design (PD) is a staple of HCI research \cite{muller1993participatory}, facilitating the design of effective solutions for a specific community while gaining a deep understanding of its stakeholders. The focus in PD of valuing the opinions and perspectives of users as experts \cite{schuler_participatory_1993} 
% In recent years, the tech and social work sectors have awakened to the importance of involving real users in designing and implementing digital technologies, developing human-centred design processes to iteratively design products or technologies through user feedback 
has gained importance in recent years \cite{storer2023reimagining}. Responding to criticisms and failures of past AI tools that have been implemented without adequate involvement and input from actual users, HCI scholars have adopted PD approaches to design predictive tools to better support human decision-making \cite{lehtiniemi_contextual_2023}.
% ; accordingly, in social service, a line of research has begun studying and designing for human-AI collaboration with real-world users (e.g. \cite{holten_moller_shifting_2020, kawakami2022improving, yang_unremarkable_2019}).
Section \ref{subsec:relatedworkaiuse} shows a clear need to better understand SSP perspectives when designing and implementing AI tools in the social sector. 
Yet, PD research in this area has been limited. \citeauthor{yang2019unremarkable} (2019), through field evaluation with clinicians, investigated reasons behind the failure of previous AI-powered decision support tools, allowing them to design a new-and-improved AI decision-support tool that was better aligned with healthcare workers’ workflows. Similarly, \citeauthor{holten_moller_shifting_2020} (2020) ran PD workshops with caseworkers, data scientists and developers in public service systems to identify the expectations and needs that different stakeholders had in using ADS tools.

% Indeed, it is as Wise \cite{wise_intelligent_1998} noted so many years ago on the rise of intelligent agents: “it is perhaps when technologies are new, when their (and our) movements, habits and attitudes seem most awkward and therefore still at the forefront of our thoughts that they are easiest to analyse” (p. 411). 
Building upon this existing body of work, we thus conduct a study to co-design an AI tool \textit{for} and \textit{with} SSPs through participatory workshops and focus group discussions. In the process, we revisit many of the issues mentioned in Section \ref{subsec:relatedworkaiuse}, but in the context of novel generative AI systems, which are fundamentally different from most historical examples of automation technologies \cite{noy2023experimental}. This valuable empirical inquiry occurs at an opportune time when varied expectations about this nascent technology abound \cite{lehtiniemi_contextual_2023}, allowing us to understand how SSPs incorporate AI into their practice, and what AI can (or cannot) do for them. In doing so, we aim to uncover new theoretical and practical insights on what AI can bring to the social service sector, and formulate design implications for developing AI technologies that SSPs find truly meaningful and useful.
% , and drive future technological innovations to transform the social service sector not just within [our country], but also on a global scale.

 % with an on-the-ground study using a real prototype system that reflects the state of AI in current society. With the presumption that AI will continue to be used in social work given the great benefits it brings, we address the pressing need to investigate these issues to ensure that any potential AI systems are designed and implemented in a responsible and effective manner.

% Building upon these works, this study therefore seeks to adopt a participatory design methodology to investigate social workers’ perspectives and attitudes on AI and human-AI collaboration in their social work practice, thus contributing to the nascent body of practitioner-centred HCI research on the use of AI in social work. Yet, in a departure from prior work, which have largely focused on existing ADS tools (e.g., AFST) and were situated in a Western context, our paper also aims to expand the scope by piloting a novel generative AI tool that was designed and developed by the researchers in partnership with a social service agency based in Singapore, with aims of generating more insights on wider use cases of AI beyond what has been previously studied.

% i may think 'While the current lacunae of research on applications of AI in social work may appear to be a limitation, it simultaneously presents an exciting opportunity for further research and exploration \cite{dey_unleashing_2023},' this point is already convincing enough, not sure if we need to quote here
% I like this end! it's a good transition to our study design, do we need to mention the localization in intro as well? like we target at singapore

% Given the increasing prominence and acceptance of AI in modern society, 

% These increased capabilities vastly exacerbate the issues already present with a simpler tool like the AFST: the boundaries and limitations of an LLM system are significantly more difficult to understand and its possible use cases are exponentially greater in scope. 

% Put this in discussion section instead?
% Kawakami et al's work "highlights the importance of studying how collaborative decision-making... impacts how people rely upon and make sense of AI models," They conclude by recommending designing tools that "support workers in understanding the boundaries of [an AI system's] capabilities", and implementing design procedures that "support open cultures for critical discussion around AI decision making". The authors outline critical challenges of implementing AI systems, elucidating factors that may hinder their effectiveness and even negatively affect operations within the organisation.


% Is this needed?:
% talk about the strengths of PD in eliciting user viewpoints and knowledge, in particular when it is a field that is novel or where a certain system has not been used or developed or tested before

==> sections-old/3_stage1design.tex <==
\section{Stage 1: Preliminary Interviews}
\label{sec:stage1design}


% \begin{table}
%   \caption{Workshop Participants from Agency A and Agency B}
%   \label{tab:workshopParticipants}
%   \begin{tabular}{cc|cc}
%     \toprule
%     \multicolumn{2}{c|}{\textbf{Agency A}}&\multicolumn{2}{c}{\textbf{Agency B}} \\
%     \midrule
%     Code&Role&Code&Role\\
%     \midrule
%     \multicolumn{2}{c|}{Group 1}& \multicolumn{2}{c}{Group 1} \\
%     \midrule
%     TS1 & Senior Social Worker & CD1 & Director\\
%     TS4 & Social Worker & CY1 & Youth Work Services\\
%     TS5 & Social Worker & CY2 & Youth Work Services\\ 
%     TS6 & Social Worker & CY3 & Youth Work Services\\
%     TS7 & Social Worker & CP1 & Youth Projects\\
%     && CP2 & Youth Projects\\
%     && CP3 & Youth Projects\\
%     \midrule
%     \multicolumn{2}{c|}{Group 2}&\multicolumn{2}{c}{Group 2} \\
%     \midrule
%     TD1 & Executive Director & CC1 & Counsellor\\
%     TD2 & Senior Director & CC2 & Counsellor\\
%     TS2 & Social Worker & CC3 & Counsellor\\
%     TS3 & Social Worker & CC4 & Counsellor\\
%     TP1 & Psychologist & CP4 & Youth Projects\\
%   \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}
%   \caption{Other Participants from Agency A and Agency B}
%   \label{tab:otherParticipants}
%   \begin{tabular}{ccl}
%     \toprule
%     Code&Role\\
%     \midrule
%     \multicolumn{2}{c}{\textbf{Agency A}} \\
%     \midrule
%     TS8 & Social Worker\\
%     TS9 & Social Worker\\
%     TS10 & Social Worker\\
%     \midrule
%     \multicolumn{2}{c}{\textbf{Agency B}} \\
%     \midrule
%     CC5 & Counsellor\\
%   \bottomrule
% \end{tabular}
% \end{table}

% \begin{figure}
% \begin{minipage}{.5\textwidth}
\begin{figure}
    \centering
    \includegraphics[scale=0.25]{images/masked participants + postits.png}
    \caption{(Left) Workshop participants (faces masked for review); (Right) Notes generated by participants}
    \Description{(Left) A picture of workshop participants with faces masked for review; (Right) Post-It notes generated by participants.}
    \label{fig:workshops}
\end{figure}
% \end{minipage}%
% \begin{minipage}{.5\textwidth}
\begin{table}
  \caption{Workshop Participants from Agency A and Agency B}
  \label{tab:workshopParticipants}
  \begin{tabular}{cc|cc}
    \toprule
    \multicolumn{2}{c|}{\textbf{Agency A}}&\multicolumn{2}{c}{\textbf{Agency B}} \\
    \midrule
    Code&Role&Code&Role\\
    \midrule
    TS1 & Snr Social Worker & CD1 & Director\\
    TS2 & Social Worker & CY1 & Youth Work \\
    TS3 & Social Worker & CY2 & Youth Work \\ 
    TS4 & Social Worker & CY3 & Youth Work \\
    TS5 & Social Worker & CP1 & Youth Projects\\
    TS6 & Social Worker & CP2 & Youth Projects\\
    TS7 & Social Worker & CP3 & Youth Projects\\
    TS8 & Social Worker & CP4 & Youth Projects \\
    TS9 & Social Worker & CC1 & Counsellor \\
    TS10 & Social Worker & CC2 & Counsellor \\
    TD1 & Exec. Director & CC3 & Counsellor\\
    TD2 & Snr Director & CC4 & Counsellor\\
    TP1 &  Psychologist & CC3 & Counsellor\\
    && CC4 & Counsellor\\
    \Description{Table describing workshop Participants from Agency A and Agency B. There are 13 participants from Agency A, mostly social workers, and 14 participants from Agency B, a mix of youth workers, youth project workers, and counsellors.}
  \bottomrule
\end{tabular}
\end{table}
% \end{minipage}
% \end{figure}


We adopt a two-stage PD process for a comprehensive and structured understanding of the role of social work in AI. In Stage 1, we conduct formative PD workshops to shape our understanding of the interplay between AI and social work. The knowledge gained here sets the foundation for a more empirical, in-depth investigation in Stage 2 (Section \ref{sec:stage2design}).

We began with two workshops (Fig. \ref{fig:workshops}) with two social service agencies, A and B, in November 2023. This provided a high-level understanding of the social service sector pertaining to possible AI solutions and possible associated implementation challenges. A total of 27 SSPs were involved, hailing from different roles and experience levels (Table \ref{tab:workshopParticipants}),
% came from a variety of roles within their agencies (Table \ref{tab:workshopParticipants}) and worked with different groups of clients (e.g. youths, families, and adult clients). 
giving us a wide range of perspectives to draw upon. 

Each workshop lasted around 90 minutes, comprising a  briefing and discussion session. In the briefing, we introduced LLMs in the form of ChatGPT\footnote{At the time of the workshops (October 2023), ChatGPT was the main LLM widely accessible to the public.}. We demonstrated AI's strengths (e.g., brainstorming, ideation \cite{gero2023social, shaer2024ai}, summarisation \cite{wang2023chatgpt}, formatting and rewriting of text \cite{bhattaru2024revolutionizing}) and weaknesses, including hallucination \cite{maynez2020faithfulness} and limited context windows \cite{liu2024lost}. This ensured that all participants, including those with only a cursory understanding or awareness of ChatGPT\footnote{ChatGPT had been available for around 10 months at this point. Some workers had tried using it, even experimenting with it for their work, while others had never used it themselves.} had a baseline understanding of LLMs.

% just to clarify, so here is like before conducting the interview, there is a session to inform participants about the potential use of LLM? I wonder if this will give a preconception to them when answering the questions regarding LLM's pros/cons? As I remembered when I was coding there was a code called ideation/summarization/formatting haha. Will it be affected by this preconception? I wonder if it would be better to be a subsection..?

Next, we split participants into tables of 4-6 people each for small-group discussions. Here, we sought to encourage participants to freely express their thoughts and build on one anothers' ideas \cite{bonnardel2020brainstorming}. Participants were given stacks of Post-Its and asked a series of questions. For each question, they spent around five minutes writing their responses on individual Post-Its. Then, they pasted their Post-Its on a board and clustered similar ideas together, allowing common themes to emerge. To kickstart the discussion with more familiar topics, we asked the participants about their work: \textit{"What does a day at work look like for you?"}, \textit{"What difficulties have you recently faced in your work?"}. We then brought AI into the picture:\textit{ "How can AI help you in your work?"}, \textit{"What expectations do you have for an AI-powered social service tool?"}. Having elicited some ideas, we then introduced two rounds of 6-8-5 sketching where participants quickly drew out concepts of possible AI tool that could help them. Finally, we asked, \textit{"What are some concerns you might have with using AI in your work?"}.  % just to confirm, the procedure of stage 1 is like: basic knowledge about LLM -> participants are given some predefined questions -> start interview -> merge the answers directly WITH the participants? Looks like it can be unpacked more later

After the workshops, the researchers transferred the physical Post-Its to a Miro board for further analysis, and deduced themes from the clustering done during the workshops. The main findings are presented in the next section.

% Due to the iterative nature of our research process, these later sessions served to both further ideate and critique potential solutions, and also test the concrete prototypes developed at that stage. We include the former as part of our discussion here, and leave the latter for a later part of the paper.

% We start by summarising some common difficulties that plague social workers in their work. We then present how participants felt that AI could help address these issues. Finally, we discuss the potential for AI to negatively affect organisational stability in a social work agency, and ways to begin understanding this complex issue.



==> sections-old/4_stage1findings.tex <==
\section{Preliminary Findings}
\label{sec:preliminaryfindings}

We categorise our findings into three main themes: Difficulties faced by SSPs in their daily work, possible AI-assisted solutions, and potential risks of using AI systems.

% Comment: Below are the themes that discovered WITH participants right? If it will be better to write an overview at first?

\subsection{Difficulties in Social Service Practice}
\label{sec:stage1difficulties}

% The most common frustration that emerged was documentation. Across the social work workflow, the constant need to document "anything and everything" (TS3) is a major timesink. Reports must be written in a systematic manner in many different categories like bio-psychological scales (TS2) or numerous risk factors (TS3). Further, the same content may need to be repackaged for different stakeholders (TD2, TS3) like colleagues or other agencies, creating tedious duplicate work. Beyond repackaging and reformatting information, documentation also involves analysis of client profiles. Workers may need to synthesise information from many pages of case notes to formulate assessments and justify a certain judgement (TS3), a cognitively challenging task. 

% Beyond being time-consuming, documentation is also not a task that is in the innate skillset of a social worker. Senior personnel desired greater incorporation of theoretical concepts in their staff's reports (TD1, TD2), observing them "knowing what to do" in practice but being unable to translate that well into writing (TD1). This is especially relevant when writing assessments of a client, where workers ideally select from a "toolkit" of frameworks to produce a justified and sound assessment (TS3).

% Aside from documentation, case formulation is another key step integral to case work. Piecing together disparate information from across many pages of case notes is time-consuming and prone to workers inadvertently missing certain key information (TD1). This is particularly tricky during a live session with the client, where the non-linear process of information discovery (CC2) means workers are constantly trying to organise their "all over the place" (CC5) thoughts to understand a case holistically before proceeding to ask the client the most pertinent questions. This may inadvertently cause them to miss certain key insights or red flags (TS2, TD1) only evident from looking at the gathered information as a whole.

Echoing past sentiments \cite{singer_ai_2023, tiah_can_2024}, participants cited the \textit{need to document "anything and everything"} (TS3) as a major pain point. SSPs have to write systematic reports in different structured formats (e.g. bio-psychological scales (TS2), risk factor assessments (TS3)) and repack the same content for different stakeholders (TD2, TS3) like colleagues or other agencies, creating tedious duplicate work. Additionally, some SSPs struggle with putting their ideas into text, "knowing what to do" in practice but being unable to translate that well into writing (TD1). This results in a lack of ability to incorporate theoretical concepts in reports, something noted particularly by senior personnel (TD1, TD2). 
% This is especially relevant when writing assessments of a client, where workers should ideally select from a "toolkit" of frameworks to produce a justified and sound assessment (TS3). 
% MH: difficulty 1: doc - interesting! just tried to summarize the mainpoints: 1) reduce time; 2) help junior staffs to proofread the report writing? Will it be better to seperated to two paragraphs..?

Participants also noted the \textit{challenges in case formulation}, the synthesising of information to craft assessments and justify a certain judgement (TS3). Piecing together disparate information across many pages of case notes is cognitively challenging and time-consuming (TD1). This is especially tricky during direct interaction with a client, where the non-linear process of information discovery (CC2) leaves workers constantly trying to organise their "all over the place" (CC5) thoughts to understand a case holistically before proceeding to ask the client the most pertinent questions. This may inadvertently cause them to miss certain key insights or red flags (TS2, TD1) only evident from looking at the gathered information as a whole.

\subsection{Possible Solutions}
\label{sec:stage1solutions}

Having elucidated these difficulties, participants floated numerous ideas for how AI could help with these issues. Many participants expressed a desire for a tool to help with \textit{manual labour}- for example, turning point-form notes into formal reports (CP1, CP2, CC1, TS2). TD1 shared how SSPs frequently used the "5Ps" framework\footnote{Presenting problem, Predisposing factors, Precipitating factors, Perpetuating factors, Protective factors} to organise case information into different, logically linked categories to aid subsequent analysis. This is one possible, largely menial and procedural task that an LLM could perform with high accuracy. Other forms of documentation mentioned, like the Data, Intervention, Assessment, Plan (DIAP) or Bio-Psychosocial-Spiritual (BPSS) formats, were also common report structures that could be automatically generated. 

More cognitively-intensive, \textit{mental labor} tasks were also considered, such as the generation of assessments (TS3, TS4, TS6, TS7). This requires fitting a client's information into theoretical frameworks to produce well-grounded assessments and analyses. AI tools could improve both the speed at which relevant information is synthesised and categorised, and the quality of the output through use of technical, industry-standard terms, something that is often lacking in many SSPs (TD1, TD2). Another critical task is intervention planning, where workers follow established models like Cognitive Behaviour Therapy (CBT) or Solution-Focused Brief Therapy (SFBT) and craft a plan for their clients based on the guiding steps in each model. An AI tool could allow rapid generation of numerous possible interventions (CP1), leaving the user to pick and choose from the suggestions offered (TD1).


\subsection{Areas of Risk}
\label{sec:stage1risks}
In line with past work on the dangers of AI adoption [cite], participants echoed certain concerns about the use of AI tools. Privacy of client data was uniterally mentioned by all, a universal concern core to the social sector. Storage of personal client information (TS3, TP1) was a particular worry, and TS1 noted the possibility of workers entering sensitive information into a system by mistake. On the staff competency front, a common concern was the consequences of AI taking on an increasing part of the worker's job scopes. Specifically for analytical or ideative tasks, some seniors (TD1, TD2, TS1) were concerned about the loss in critical thinking skills of junior workers who might become overreliant on the tool to perform their work for them. Multiple participants also raised the possibility of inaccurate outputs from an AI system, particularly risky when less experienced workers fail to tell when the AI's output might be suboptimal and proceed to adopt its suggestions anyway. 
% 1) data privacy; 2) overreliance; 3) inaccurate output (participant identifiers are missed for 3 (?)


% This doubtless was influenced by our intial presentation on generative AI capabilities, where we showed an example of an LLM summarising and reformatting case notes. 

% \subsection{Research Questions and Testing Goals}

% From the above, we derive the following research questions.

% First, while many workers suggested they would be interested in AI automation tools, care needs to be taken to design such tools in a manner that is useful to them. Developing a tool that does not fit in their workflow or give outputs that are what they are looking for is pointless.


% \textbf{\textit{RQ1}}: What kind of AI tools do social workers find useful in their daily lives? How can they use these in their daily work?


% Besides non-useful outputs (possibly a system designer flaw), AI tools may also make more micro-level mistakes, such as by making topically relevant, yet incorrect or suboptimal suggestions. The ability of LLMs and other AI systems to handle social work-related queries is, to our knowledge, almost entirely unexplored.


% \textbf{\textit{RQ2}}: How accurately can modern AI tools handle these tasks?


% Given a tool that provides relevant, high-quality aid to social workers, the question shifts to how these tools should be most effectively implemented in and throughout an agency, maximising benefits while minimising harm.


% \textbf{\textit{RQ3}}: How do staff in different positions in the organisation use or think about the tool differently? What different user requirements might they have?


% \textbf{\textit{RQ4}}: How should staff in different positions in the organisation use or be given access to the tool differently? How can the tool serve to complement while not replacing human social workers?

==> sections-old/5_stage2design.tex <==
\section{Stage 2: Prototype and User Testing}
\label{sec:stage2design}

The above workshops gave us an understanding of what a relevant and useful AI system to aid SSPs might look like. To empirically evaluate how well the ideas raised by participants would translate to real use, we built a prototype tool incorporating many of the proposed solutions (Section \ref{sec:stage2systemdesign}), and tested these out with another group of SSPs (Section \ref{sec:stage2fgddesign}). 

\subsection{System Design}
\label{sec:stage2systemdesign}

\begin{figure}
    \centering
    \includegraphics[scale=0.25]{images/prototypetool.png}
    \caption{Prototype AI Tool}
    \Description{A screenshot of our prototype AI tool. It has a text box for entry at the top, a list of radio buttons to select output modalities, a text box for extra instructions to the model a user might want to input, and a "generate" button.}
    \label{fig:tool}
\end{figure}

Based on the opportunities and concerns identified above, we created a prototype assistant tool (Figure \ref{fig:tool}) and tested it out in a series of focus group discussions (FGDs). Our design approach was to explore the full range of possible ways in which workers could use AI for help. We positioned the prototype system as a \textit{general purpose AI assistant for social service practitioners}, where users could present the system with as little or as much information about a client as they wished, before asking it to generate various outputs according to what they needed. % that's pretty clear! Will there be an interface of it? Also a bit not sure - so the function modules of this prototype is implemented based on stage 1 right? Will it be necessary to unpack how we correspond the participant's envision to the function module?

The tool comprised an input text box for users to enter details about their client and a number of different types of output options. Users could select an output option based on a desired use case, then click a "generate" button to produce an LLM-written\footnote{OpenAI GPT-4 Turbo, gpt-4-1025-preview} response. These output options addressed various difficulties in social work, such as manual labor and mental labor, (Section \ref{sec:stage1difficulties}) and simulated potential uses addressing these difficulties (Section \ref{sec:stage1solutions}). In response to complaints about manual work, the tool offered options to rewrite workers' rough notes into various organization-wide formats (e.g. BPSS\footnote{Bio-Psychological-Spiritual - a recognised standard for client screening}, DIAP\footnote{Data, Intervention, Assessment, Plan - a standard post-client meeting report format}, Ecological, 5Ps). Users also raised points about assessments, case conceptualization, and ideation. We included options for strength, risk, and challenge assessments, following common social service practices \cite{rooney2017direct}. Finally, we added options to generate client intervention plans according to three common theoretical models: CBT\footnote{Cognitive Behavioural Therapy}, SFBT\footnote{Solution-Focused Brief Therapy}, and Task-Centered interventions. 

An important consideration was ensuring the generalisability of our findings, making sure our system and subsequent discussions adequately represented the vast possibilities of AI use cases, and not being limited to exploring a particular LLM in a specific configuration. We address this by noting the difference between areas that other or future AI systems may improve in, such as reasoning and knowledge, and those that they are unlikely to, such as being able to account for a user's (or client's) contextual factors. It is the latter that we focus our investigation on: Given an AI system is ultimately constrained by its training dataset, what are the possibilities with such systems and what are the potential downsides?

\subsection{Focus Group Discussion Design}
\label{sec:stage2fgddesign}

We tested the prototype system in a round of Focus Group Discussions (FGD), where we simulated a contextual inquiry process \cite{holtzblatt2017contextual} by asking participants to walk us through their use of our tool and explain their thought processes along the way. We also encouraged them to point out weaknesses or flaws in the system and suggest potential improvements. We structured the FGDs for two main purposes: 1) to understand the \textit{opportunities} of AI use in social work (Section \ref{sec:stage2designuses}), based on the opportunities identified in Section \ref{sec:stage1solutions}; and 2) to identify the \textit{challenges} of using AI in this sector (Section \ref{sec:stage2designrisks}), based on the concerns raised in Section \ref{sec:stage1risks}.

\begin{table}
  \caption{Focus Group Participants from Agency A}
  \label{tab:thkMayParticipants}
  \begin{tabular}{cc|cc|cc|cc|cc}
    \toprule
    \multicolumn{2}{c|}{\textbf{Centre 1}}&\multicolumn{2}{c|}{\textbf{Center 2}}&\multicolumn{2}{c|}{\textbf{Center 3}}&\multicolumn{2}{c|}{\textbf{Center 4}}&\multicolumn{2}{c}{\textbf{Management}}\\
    \midrule
    Code&Role&Code&Role&Code&Role&Code&Role&Code&Role\\
    \midrule
    \multicolumn{2}{c|}{Group 1}& \multicolumn{2}{c|}{Group 3}& \multicolumn{2}{c|}{Group 4}& \multicolumn{2}{c|}{Group 7}&\multicolumn{2}{c}{-}\\
    \midrule
    W1 & Social Worker & S4 & Supervisor & S6 & Senior SW & S8 & Senior SW & D1 & Director*\\
    W2 & Social Worker & S5 & Supervisor & W5 & Social Worker & S9 & Senior SW & \multicolumn{2}{c}{\textit{*Observer in}}\\
    W3 & Social Worker & W4 & Social Worker &&& S10 & Senior SW & \multicolumn{2}{c}{\textit{multiple sessions}}\\
    \midrule
    \multicolumn{2}{c|}{Group 2}&\multicolumn{2}{c|}{}&\multicolumn{2}{c|}{Group 5}&\multicolumn{2}{c|}{Group 8} \\
    \midrule
    S1 & Supervisor &&& S7 & Senior SW & W11 & Social Worker\\
    S2 & Supervisor &&& W7 & Social Worker & W12 & Social Worker\\
    S3 & Supervisor &&& W8 & Social Worker & W13 & Social Worker\\
    \midrule
    &&&& \multicolumn{2}{c|}{Group 6}\\
    \midrule
    &&&& W9 & Social Worker\\
    &&&& W10 & Social Worker\\
    &&&& C1 & Snr Counsellor\\
  \bottomrule
  \Description{Table describing Focus Group Participants from Agency A. There are 8 groups from 4 different centres, plus a director classified under "Management".}
\end{tabular}
\end{table}

We conducted the FGDs in groups of 2-4 SSPs from Agency A.
%\footnote{Agency B opted to explore a different LLM-based social service solution. We discuss this work in another paper (forthcoming).}. 
We sought a mix of workers of varying seniorities (Table \ref{tab:thkMayParticipants}), to gain perspectives across different organizational levels. We held a total of 8 sessions totaling 24 participants. Each session averaged 45-60 minutes in length and was audio-recorded for transcription and analysis. 



\subsubsection{Understanding Opportunities with AI}
\label{sec:stage2designuses}

The main goal of the FGDs was to simulate real-life usage of our system. We asked participants to bring along real case notes from recent clients they had worked with, anonymizing them beforehand to remove any personal information. We explained the various functions of the system, then told participants to imagine themselves using it to help with the cases they had on hand. As participants brought along different types of case files (e.g., rough short-hand notes, complete reports, intake files), this allowed us to explore a range of different use cases, from generating reports for documentation to planning future sessions or interventions for the client.

We also learned early on that case supervision by senior workers was a key means of addressing the difficulties faced by junior workers and encouraging worker development. We therefore sought to understand how AI could play a collaborative role in the supervision process. In sessions with supervisors present, we asked these more senior workers how they felt the various functions of the system could aid them in their discussion of cases with their supervisees. 

% just have a general question emerged when i read here: why two stage? anywhere explained this? I feel the workshop is also used to understand what is expected by SW? What's the main difference between FGD and workshop? I feel maybe need to say 1-2 sentence somewhere? Is that because something will be found ONLY AFTER a real prototype is there?

% With state-of-the-art LLMs as a platform, we sought to elucidate the specific areas in which AI systems fall short in providing the required level of specificity in social work cases. 
% oh maybe a silly question is: I haven't read a paper that use FGD as its main research method, but I wonder will it require describing the FGD protocol? Like specifically what questions are asked?

% is then offered two sets of analysis, roughly corresponding to the user needs of documentation and ideation. The four options in the first row - Ecological, Strengths, Risks, 5 Ps - are some of the most common ways of analysing case information that came up throughout our discussions. These can be used either during a session with a client, to quickly organise their notes and take stock of their current progress, or after a session when writing a report in a certain format. The three options below - Task-Centered, CBT, SFBT - are three major intervention modalities \cite{rooney2017direct} that collectively cover a wide range of client types. These can help social workers review their options for selecting a suitable plan for their client, or easily selecting and combining pieces of each potential plan to form a new, hybrid one.

\subsubsection{Understanding Challenges with AI}
\label{sec:stage2designrisks}

On the other hand, we also sought to understand the possible challenges of using AI tools in social work. In testing the tool, we asked participants to review the quality of the outputs, compare them to their own, and identify areas where they would fall short of expectations or fail to be useful in their daily work. We note that while our platform is based on GPT-4, a general purpose model not tuned for social work analysis\footnote{Specialised AI systems for social work case management do exist (e.g. \cite{socialworkmagic2024, caseworthy2024}, but these are focused on user experience and do not provide greater insight than vanilla GPT; furthermore, \cite{socialworkmagic2024} advises users to take its assessments and suggestions as only a starting point, which aligns with how we position our tool.}, our aim was not to discover the specific weaknessses of GPT-4 or any LLM in particular. Rather, it was to understand what participants perceived to be good outputs from an AI system, and in the process understand how they might be affected by any possible shortcomings of such a system. % I actually feel the footnote here is pretty important at the first glimpse haha

We also explored some of the wider effects of AI use. Participants were asked about potential overreliance on the tool and the possibility of becoming overly trusting of the system's output. Senior workers in particular were asked about how they perceived junior workers new to the sector having such a system to help them with their daily work.
% so the novelties lied in: test vanilla GPT and analyze the need/requirement/concern from users, rather than design a new non-generic tool to address these concern?

% This interface was meant to mimic what a actual assistant tool used by social workers might look like. A large, free-text text box at the top of the screen allows users to put large sets of case notes in. 

% \subsection{Remote Testing}

% In addition to the above, we tested the same tool on a wider scale within THK. These staff members were given access to a limited set of functionalities of the tool, specifically those that had been identified as having more reliable outputs, and told to use them in their daily work. From this we collected more data on the tool's performance and its users behaviours.

\subsection{Data Analysis}
\label{sec:stage2analysis}

To analyze the session transcripts, we performed qualitative thematic analysis \cite{braun2006using}. Qualitative thematic analysis is a method for identifying and analyzing key patterns and themes within interview and focus group data that affords a flexible and iterative coding process \cite{braun2006using}, making it particularly suited to the iterative nature of PD studies like this one. Due to the nascence of AI in social service sector and the paucity of existing theoretical frameworks specific to the context of our study, we adopted an inductive, bottom-up approach of coding, which allowed us to uncover emergent themes in a data-driven manner and surface the latent thoughts, feelings and attitudes of SSPs in their own voice, rather than attempting to fit the data within a preexisting framework or being influenced by researchers' prior analytic preconceptions. 

Coding of the transcripts was carried out sequentially and iteratively. First, four researchers independently coded two transcripts, and met to discuss and share the codes. Subsequently, two researchers then independently developed a codebook based on identified codes, and met to combine the two into a unified codebook of themes and subthemes. The codebook was shared with the other two researchers alongside explanatory memos, and used to code the remaining six transcripts, which were equally divided among all four researchers, with at least two researchers coding each transcript. The researchers then met two additional times to discuss the codes and resolve disagreements, until consensus was met. Finally, two researchers met in multiple rounds to collaboratively revise and refine the codes, as new themes were discovered and old ones were combined or retired. These themes form the final framework described below. % do we need to spell out the coding procedure here? Like how many coders, open discussions, etc

==> sections-old/6_stage2findings.tex <==
\section{Findings}
\label{sec:stage2findings}

% Based on the codebook and themes, a final framework was developed, summarizing the Values, Requirements, and Attitudes that social workers have towards the application of AI tools in the social work practice.

\begin{figure}
    \centering
    \includegraphics[scale=0.15]{images/ai in ss.png}
    \caption{Framework Situating AI in the Social Service Sector}
    \label{fig:situatingAI}
    \Description{An image showing our framework situating AI in the social service sector. There are three columns of subthemes: Ethos, comprising Ethics Experience, and Expertise; Attitudes, comprising Apprehension, Ambivalence, and Acceptance; and Considerations, comprising Care, Context, Control, and Collaboration.}
\end{figure}

We propose a framework encapsulating the fundamental place of AI in the social sector (Figure \ref{fig:situatingAI}). We term this the \textit{\textbf{ACE}} framework, comprising \textit{\textbf{A}ttitudes} of SSPs towards AI, \textit{\textbf{C}onsiderations} for systems congruent with SSPs' core identities, and the \textit{\textbf{E}thos} of SSPs and what matters to their profession in the \textit{context of AI systems}.

Each of the three themes consist of 3-4 subthemes. Under \textbf{E}thos, we discuss SSPs' \textit{\textbf{e}thics} (core values and beliefs), \textit{\textbf{e}xperience} (human touch and instinct), and \textit{\textbf{e}xpertise} (knowledge and skills), which are fundamental to the profession of social work. These in turn inform SSPs' \textbf{A}ttitudes towards AI, which are characterised by a combination of \textit{\textbf{a}cceptance}, openness and amazement towards AI, \textit{\textbf{a}pprehension} and caution about AI, and \textit{\textbf{a}mbivalence} and uncertainty towards AI. Finally, these ethos and attitudes contribute towards key \textbf{C}onsiderations for AI systems in the social service sector, emphasising \textit{\textbf{c}are} for safety and privacy, \textit{\textbf{c}ontext} of case and clients, \textit{\textbf{c}ontrol} by users, and \textit{\textbf{c}ollaboration} between humans and AI. In the following subsections below, we will expand upon each of the themes and subthemes in greater detail.

\subsection{Ethos: What matters to social service practitioners?}
\label{subsec:ethos}

We first consider the principles core to SSPs and their profession. SSPs espouse a set of core values and competencies \cite{rooney2017direct}; any use of AI in the field must therefore respect these values to achieve acceptance and ethical usage. Here, we describe three main subthemes: \textbf{E}thics, \textbf{E}xperience, and \textbf{E}xpertise.

\subsubsection{Ethics: Values \& Beliefs}
\label{subsubsec:ethics}

A foremost concern amongst participants was aligning AI use with the key ethical principles of the profession \cite{difranks2008social}. Two main areas of concern emerged: safety and privacy.

\begin{quote}
\textit{"At Agency A, we think a lot about the safety and risk concerns first."} (W2)
\end{quote}

The first was the primacy of the \textit{safety and risk of clients}. 
% Safety is a crucial dimension given the sensitive nature social work cases. This leads 
SSPs were "very particular about... risks," (S9), treating it as their top priority (W1, S10) and "at the front" for all client interventions and risk assessments (S2, S9); preventing imminent physical and psychological harms such as incarceration, abuse, and addiction, were cited as "non-negotiables" and primary risk factors (W2). Participants emphasised that in any AI system, "risk and safety... is basically something that should be there for all kinds of output... in every single case" (S2). 
% Ensuring client safety and mitigating risks is therefore a core requirement in all facets of social service work, including AI systems.

% underpinning all AI systems in social work, both in terms of AI-generated assessments and outputs, and the necessity of AI tools in being able to prioritize and safeguard the safety and well-being of clients.

% while auditors also pay close "attention to much of it" (S9).

\begin{quote}
\textit{"It's in our code of ethics... to protect as much [client information] as we can."} (D1)
\end{quote}

SSPs also expressed concerns about \textit{data privacy and confidentiality}. 
% Social workers discussed their dilemma with 
These are cornerstones of the social service profession \cite{dickson1998confidentiality}, but are also gray areas fraught with ethical ambiguity and uncertainty (D1). Social service agencies accumulate vast amounts of sensitive personal information about clients over years of interactions.
% from years of session notes and case reports. These contain highly personal information about clients' mental health, socioeconomic status, interpersonal relationships and more. 
Participants worried about leaking this information, such as by "accidentally putting a name inside the system" (W8), and questioned whether it was "safe enough for us to put a name" (W8) or sensitive topics like suicide and rape (D1) into the AI system directly, and whether there was a "need to change the [client's] name" (W5).
% , reflecting their concerns on client privacy. 

\subsubsection{Experience: Human Touch and Instinct}
\label{subsubsec:experience}


    % \textit{"I think we still need human skills... maybe we just need a human connection."} (D1) 
    % \textit{"We still need the human factor."} [W8]
% \end{quote}

\label{sec:perception}
Our second theme relates to the innately human element of social work. Real-life work often deviates from textbook procedures; SSPs must thus be able to perceive a client's situation through instinctive deductions empowered by years of experience and training. Participants repeatedly emphasised the "human skills" (D1) and "human factor" (W8) required to talk to, connect with, and understand a client (S7).
% This is perhaps the one area in which AI systems might never fully replace humans (D1).   
% An obvious skill here is the actual ability to talk to clients during sessions (S7), which ultimately determines the effectiveness of a social worker in connecting with a client. Beyond that, however, being able to understand a client's situation and reactions comprises many more aspects.

% The theme of adaptability related to the core social work value of treating every client as a unique individual with distinct circumstances and needs. 

\begin{quote}
    \textit{"This family, this mother is really, wow, you know... [this workshop] will not work."} (W5)
\end{quote}

The instinct to \textit{recognise when and why to choose certain interventions} for a client is key. Interventions that are sound in theory may turn out to be unsuitable, such as in the above quote by W5 where he recognised the reluctance of a client to embrace outside help, making a parenting workshop inappropriate, or when W11 judged the lower intellectual capacity of their client to make CBT unsuitable. Furthermore, given the dynamic nature of social service practice, the instinct acquired by SSPs through experience is crucial for tailoring assessments dynamically based on individual client needs, as highlighted by the quote by S10.
% to coming up with case assessments and interventions, which require an intrinsic human touch and dynamism to tailor and personalize to clients' individual needs. Such human experience and ability is therefore difficult to be easily replicated by an AI system, which is generally more rigid and adheres to a certain set of rules and training data.


\begin{quote}
    % \textit{"Assessment is very dynamic...[AI can provide] guidelines but you also need to customize it based on where your client is at and where you are at in terms of your experience and confidence."} (S10)
    \textit{"Sometimes information may suggest a symptom of a different problem." (C1)}
\end{quote}

Experience also allows SSPs to make \textit{instinctual deductions about a client}. C1 raised the example that a complaint of joint pain would normally be associated with arthritis, but if the client were a teenager (an age group not often inflicted with joint damage), they would more likely be experiencing psychosomatic pain caused by mental stress, leading to a vastly different treatment plan. While such information could be found in a medical handbook, the ability to instinctively recall the requisite knowledge and and quickly synthesise it with information about a client sets SSPs apart.

\begin{quote}
    \textit{"Many of us who have been in the sector before, probably were like,} aiyah, \textit{this won't work."} (W5)

\end{quote}

Finally, \textit{knowledge of local and cultural factors} helps SSPs make better decisions. As a seasoned industry worker, S6 knew that "there are a few parenting workshops available [here in our country] and how they are structured," and that they would not "fit into the family" under her care. Such experience can only be gained through years of on-the-ground work and effectively utilized by appropriate human decision-making.

% This experience is also irreplaceable by AI: no system will be able to capture the "structure" of local parenting workshops and subsequently interpret their suitability for a client, since there is no way of representing such knowledge in digital form. 
 % This last example in particular illustrates one challenge of AI-assisted social work processes: it is not possible for any AI system to produce such an insight; the worker (W5) himself would not have noted down the relevant information that would have led to this assessment, and could therefore not possibly have entered it into any system for analysis. \textit{[Cite more here...]} 

\subsubsection{Expertise: Knowledge and Skills}
\label{sec:proficiency}

The third principle relates to the \textit{theoretical competencies} of SSPs, and how they use their knowledge and skills to most effectively help their clients.
% We analogize the theoretical knowledge of SSPs to a vast toolbox with tools for different purposes. 

\begin{quote}
    \textit{"The beauty of social work is [in] the dynamism of the interactions."} (S9)
\end{quote}

SSPs highlighted the need to \textit{react and adapt to client circumstances}. The "dynamics of the [client's] ecological system" (S9), such as a client's behaviour or living situation, mean that the resulting interventions "may change according to the need and time" (S4). S10 also referenced how "assessment is very dynamic", requiring SSPs to constantly asses the situation and adapt their intervention plans accordingly.

\begin{quote}
    \textit{"It's not one-size-fits-all." } (W13) 
        
\end{quote}

SSPs also require the \textit{ability to tailor each case to meet the unique needs}. C1 mentioned, "It really depends on.. the case... we will consider different models based on the information that we receive...", listing examples of violence, homelessness, and marital issues that she would use different assessment frameworks for, even "mix[ing] and match[ing]" theories as appropriate. W10 concurred, saying that from a given set of theories, they had to "see what fits... according to the key details of the case" and decide on an optimal course of action.

% Case conceptualization is a flexible, iterative, and dynamic process of selecting the right tools and combining them in the right order to create a pipeline that turns raw data about a client into a specialized and accurate assessment. W10 commented: "I think, for social workers, not all of us stick to just one type of modality". C1 mentioned: "It really depends on.. the case... we will consider different models based on the information that we receive... is this, say, a violence issue? Is this more of a homelessness issue? Is this more of a marital issue? So if it's a marital issue, I will select a certain different assessment. If it's a child behaviour issue, then I may want to choose maybe more of the, you know, certain developmental frameworks. I may use different- so  I mix and match to the case, to the type of case. For children, you may even use attachment theory and then you want to see what comes out." W10 followed up: "So [the theories are] there, but then you will choose according to the key details of the case. So you see what fits." Evidently, each practitioner follows a unique set of theories and approaches (W10) in conceptualizing a case, due to individual preference and differing competencies. 
% W10 noted that the intervention modalities they choose "might be slightly different based on the worker. So okay, some workers might prefer to try [intervention modalities like] SFBT approach or CBT approach… also there are workers who do [assessment techniques] like strengths, challenges [as a starting point]… because for CBT and SFBT there's also these concepts in these intervention style. So a lot of times when they do their assessments it's also based on these concepts." \textit{[Cite more quotes of participants talking about their individual preferences/competencies.]} 




\subsection{Considerations: What do social service practitioners want from AI?}
From SSPs' core values, we next discuss how these principles give rise to four key considerations of adopting AI in social service: \textbf{C}are, \textbf{C}ontext, \textbf{C}ontrol, and \textbf{C}ollaboration.

\subsubsection{Care: Privacy and Safety}

Given their emphasis on ethical treatment of clients (Section \ref{subsubsec:ethics}), participants were notably fastidious on both issues: the \textit{data confidentiality} and \textit{physical safety} of clients. 

\begin{quote}
    \textit{"There's a concern... that [the AI] doesn't send home [to its servers] a lot of these personal data, right?"} (D1)
\end{quote}

With \textit{confidentiality}, a recurring concern was how much client information could be entered into the AI tool (D1, W5, W8), given the unclear ethical and legal gray areas (D1) surrounding these nascent technology. This points to multiple considerations for AI system designers: to provide \textbf{ways to obsfucate or anonymise personal information}, \textbf{clarify data storage and usage policies}, and \textbf{involve users early in the design process to ensure alignment} on confidentiality.
% The quote by D1 underscores SSPs' care and concern for the personal data protection of their clients, describing that in their use of an AI tool, they would intentionally delete and obfuscate certain sensitive or personal information so it would not be captured by the AI system. Participants were reassured that our system would not store user inputs (though OpenAI stores all requests to the GPT API for 30 days for usage monitoring and abuse prevention \cite{openai2023how}\footnote{OpenAI offers Zero Data Retention upon request, but we could not get this request approved.}), yet still felt the need to err on the side of caution and "play [it] safe" (D1). W8 felt that "name[s] shouldn't be inside" AI systems, while D1 suggested using generic initials instead. This highlights the need for systems to \textbf{clarify data storage and usage policies}, while \textbf{involving users early in the design process to ensure alignment} on confidentiality.
% These various precautions and pre-processing steps therefore highlight the care for client safety and privacy as a key consideration that SSPs had towards AI, pointing to a clear need for systems that \textbf{clearly show how any information entered will be stored and used}, but also that potential users of the tool should be \textbf{involved in discussions early and often during the design of the system} to ensure that all users are on the same page with regard to data storage and confidentiality.

\begin{quote}
    \textit{"The [risk of] violence is not highlighted. Where is the violence?"} (W1)
\end{quote}

Prioritising \textit{risks to client safety} was something else participants stressed. They expressed concern when the tool's assessments failed to emphasise (S2) or entirely omitted (W1) safety risks,
% During trials of the prototype when SSPs fed in sample case notes involving situations of domestic violence or child abuse, they were especially concerned about AI's omission of certain safety aspects, commenting that 
% "The violence is not highlighted. Where is the violence?" (W1) and that "risk isn't exactly highlighted" (S2) in AI-generated assessments. 
% They therefore feedbacked that "the risk is basically something that should be there for all kinds of output" (S2), and suggested that in future iterations of the AI tool, a useful feature would be to include "what are the non-negotiables, like no abuse, no violence, et cetera...[and] safety planning" (W2). \textit{[cite more examples here]} 
and suggested that risk indicators (S2, W4) were non-negotiables.
% We note here that while GPT-4 is generally capable at producing a great deal of relevant information about a client, it has little notion of which information is the most salient and critical, particularly in accordance to specific procedures or conventions adopted by individual organisations. 
These concerns underscore the importance of \textbf{AI tools prioritizing client safety} to avoid guiding workers toward suboptimal courses of action (S9).

% As the above suggests, the word "care" here serves double duty, for both clients and system designers. On one hand, it aptly sums up the profession as a whole: above all, SSPs are driven by care for the clients they develop relationships with. 
% Care for well- being, safety (W2), and privacy (D1) are all fundamental requirements of the profession. 
% On the other, "care" is therefore something that must be liberally applied when leveraging technologies that possess immense power and limitless use cases. Failure to do so may result in systems and user workflows that compromise core tenets of social work.

\subsubsection{Context: Client Background and History}

Experience (Section \ref{sec:perception}) strongly relates to contextual analysis in formulating cases. Numerous small details that SSPs observe interacting with clients, like personality (W5), cognition (W11), psychological state (S4), and multiple small behavioural events (D1), collectively form the contextual background that informs the assessment of a case. Context can be drawn from two sources: \textit{written} records and \textit{unrecorded} insights.

\begin{quote}
    \textit{"Cases [can be] really an accumulation of years of case recordings... [so the machine] really needs context.} (S4)
\end{quote}

\textit{Written context} is often pieced together from months or years of case notes (S4), or sometimes the "verbal diarrhea" - large amounts of unorganised information - of a new client's intake session (S6). Cleaning and analysing such raw data is time-consuming (W3) and error-prone (D1). AI systems should therefore be designed to \textbf{accept large amount of text or documents} while \textbf{thoroughly analysing all given facts and information} contained in the input, to effectively streamline processes (W1) while ensuring no critical information is missed (S6). 

% While formulating a clear view of a client's situation from these notes is imperative for effective interventions, cleaning up such overwhelming amounts of raw data and formulating them into assessments this process can be difficult and "time-consuming" (W3). This is one area where LLMs and AI, with its superior data processing and generative potential, can "definitely help" with in terms of helping social workers to "streamline [their processes] and save...time" (W1). 


% One tangible way in which this can be overcome is by designing tools capable of \textit{taking in large amounts of information}.   The ability to "plug in" (S6) tens of past reports is important to ensuring all relevant information is captured. On the other hand, access to context in past information may sometimes still be insufficient. As noted previously, social work cases involve many intangible factors that cannot be captured by AI systems. It is therefore crucial that AI system are \textit{clear and transparent on their limitations}, in order to avoid misleading users.

\begin{quote}
    \textit{"[This is your direct assessment of the family?] Yes. [But you won't necessarily detail it in the case report?] No." (W5)}
\end{quote}

With unrecorded insights, social work cases often involve intangible factors that cannot be captured by AI systems. One example is W5's quote from Section \ref{subsubsec:experience}, where the worker did not record his feeling of the client as being unreceptive to outside help. Such information, naturally, is inaccessible by the AI for its decision making. It is therefore crucial that AI system are \textbf{clear and transparent on their limitations}, in order to avoid misleading users and further encourage users to critically analyse their cases.


% The irreplaceability of the human touch in social work (Section \ref{sec:perception}) suggested the use of AI in instead developing human skills.

\subsubsection{Control: Flexibility to Customize Use}
\label{subsubsec:control}



% \begin{quote}
%     \textit{"Our assessment depends on what style we adopt... 
%     % some workers might prefer [an] SFBT approach or CBT approach... 
%     [we] take in a modality as a guide or framework that we perceive things with.
%     % .. Let's say I want to choose strength assessment but I want the SFBT interventions. Then we can look at the assessment and see, these are the strengths, so this is the proposed solutions based on SFBT approach. Then you can see the interlink between all...Also, [regarding] efficiency - you don't [have to go] back and forth on my computer; it's just one generated output report."
%     } (W9)
% \end{quote}

AI systems should complement the theoretical competencies of SSPs (Section \ref{sec:proficiency}) by offering customisable workflows instead of one-size-fits-all user flows (W13), allowing different ways of using and combining the theoretical frameworks in social service practice. 

\begin{quote}
    \textit{"Maybe put risks and strengths [side-by-side], then maybe the DIAP and the 5Ps too... then we know which [parts] we can contrast, and also get a more rounded intervention process"} (W11)
\end{quote}

Firstly, many participants suggested allowing \textit{multiple theoretical modalities in a single output}. As W9 highlighted above, SSPs have different styles and preferences in formulating cases and interventions. Therefore, participants suggested that the AI could be in-built with functions to offer such greater control and customizability, allowing users the flexibility to select and include different frameworks and modalities in the AI-generated output. This could include generating an intervention integrated with an assessment or incorporating multiple modalities within a single output (e.g., SFBT, CBT) (W9) and combining risks and strengths to assess the two in tandem (S7). Participants also proposed side-by-side outputs to compare and contrast frameworks (W11), noting that frameworks are often used together and inextricably (S10). 
% Given that many of these modalities and frameworks used by SSPs are not used in isolation of one another, but often used side-by-side to complement each other, S10 noted such combinations could be useful since certain assessment frameworks are closely or inextricably linked with others. 
% An AI system with affordances to provide higher degrees of control and customization would enable users to 
Enabling practitioners to "see the interlink between" different modalities (W9) provides a "a deeper, richer perspective" where different modalities "feed back into each other" (S7). This gives a more holistic view of each case, while improving efficiency by consolidating information in one view (S9). 
% Furthermore, a practical benefit of this is that it would allow users to access all the essential case information in a single view, without having to switch between multiple screens or files (S9), thus enhancing efficiency and saving time (which is especially useful for time-pressed SSPs, for whom every second counts).

% W9 said, "I was just thinking, would it be possible if we could do for example like an assessment and an intervention and then we generate at one shot." S7 wanted to combine the outputs for risks and strengths, to assess the two in tandem and see how one fed into the other. W10 wanted to combine "a strength assessment with an SFBT intervention to see the interlink between all because SFBT is always about building on the person's strengths". \textit{[Cite more here...]} Other participants requested parallel, side-by-side outputs. W11 suggested showing "maybe risk[s] and strengths [side-by-side], then maybe the DIAP and the 5Ps [side-by-side]... we know which [parts] we can contrast, and also get a more rounded intervention process". \textit{[Cite more here...]}. Participants showed that, while our system had a range of useful tools, participants did not want to be restricted to a single option at a time, and instead have the flexibility to pick and choose different theoretical frameworks to use.

\begin{quote}
    \textit{"If you are able to choose the people in the family, whose strength we want to look at... [that would be good]." (W5)}
\end{quote}

Secondly, participants desired \textit{control over the focus of the system's output}. Our system tended to give generic, safe answers according to its pre-programmed theoretical frameworks; participants, however, demanded more. W2 considered a "complex family with multiple issues within the family unit", and wanted to customize the tool to get intervention plans for different family members. S6 and W5 mentioned they had to "choose what they wanted" from the complete system output, and preferred to specify their needs to begin with. 
% On a more administrative level, being able to generate outputs for different purposes and audiences was also important. For example, 
Meanwhile, W13 noted the importance of tailoring social reports for different audiences, such as housing agencies or citizenship applications.
% W13 mentioned that when producing social reports, "we might categorise it as employment, financial, and so on... it depends on who we are writing the referral to. If it's for the [local housing agency], we might talk more about what the client has tried for their housing situation, whether it's for citizenship... then it's different from if I was writing to a different agency." 
These show the varied uses of AI in social services, where SSPs require control to meet specific goals, whether for interventions or documentation.
% that that SSPs may utilize AI for multiple different functions, and therefore require different degrees of control over the output in accordance to their varying needs and aims, whether for purposes of generating client interventions or for reporting purposes to different external stakeholders and target audiences. Given the multifaceted and idiosyncratic nature of the social sector, it is therefore essential that any AI systems designed for social service must be able to afford its users with control to fit their various needs and purposes. 

% Given the multi-faceted nature of social work cases, workers often need to consider multiple perspective for the same theoretical approach. W2 said, "if it's a situation of a complex family with multiple issues within the family unit itself... we have to plan not just for the client, but also for other main family members as well... to help the mother manage her issues, would we have to remove everything else and just input the mother's portion? And the biological father has a pressing issue of alcohol addiction, we have to get him help as well." 
% This indicated a desire to be able to choose multiple individuals from whose perspective the system should analyse the case. 

% The overall finding here is that social workers do not approach case conceptualization as a linear, step-by-step process. It is rather a much more dynamic approach where workers draw on various theoretical tools, almost experimenting with different ideas until they gain a sufficient understanding of a case. AI systems are perfectly suited to help with "experimenting", being able to rapidly generate content and ideas for consideration. However, their design must facilitate this experimentation by allowing sufficient flexibility in usage. We may view flexibility of input UIs as a spectrum: on one end, a single text box connected to the unlimited powers of an LLM, and on the other, a series of preset buttons and checkboxes that rigidly control the type of output. Our key finding here is that, while having certain preset options is necessary for affordance, it is also crucial that these options can be mixed, combined, and modified according to user desires. This gives social workers the level of control they need to fully harness the power of AI systems, without being hamstrung by restrictive UI options.

% Overall, greater control and flexibility improves system usefulness, while respecting the autonomy and agency of SSPs as experts in their field,  enhancing their competencies rather than reducing them to mere system operators.

% not reducing them to mere operators of a system, but instead enhancing their existing competencies workers by allowing them full control over how the tool helps them.

% In sum, context matters greatly to system designers in two ways: the context in which the system will be used by certain workers,

\subsubsection{Collaboration: Between Humans and AI}
\label{subsubsec:collaboration}

% We view collaboration through two lenses: an idea that brings great benefits when harnessed properly, but also one whose careless omission leads to many potential risks. 

% Comment from Kai Xin: I agree with Prof EJ that the "Collaboration" theme currently covers two distinct points, which may make it too wide. I revised the section to focus it purely on human-AI collaboration and cooperation, and less so on the risks (which I feel is less applicable in terms of collaboration). The original text is still retained (with % added) below.

Finally, we highlight opportunities for HAI collaboration in social service. AI can enhance casework in many ways: by picking up details workers might miss (D1), training workers' skills and knowledge (S6), and providing pointers for supervision (C1, W4).

\begin{quote}
    \textit{"I'm hoping the system as a whole can be smarter in terms of things that we might miss out [and] capture [what] people might not be aware of.
    % So for example, a client is crying all the time. Sleeping stuck and not sleeping well. So a series of these factors putting it together can raise a red flag.
    "} (D1)
\end{quote}

Firstly, AI can provide augmented intelligence in client assessments and diagnoses. D1 mentioned how AI could pick up on subtle signs that SSPs might miss due to time constraints or high caseloads: AI tools can identify patterns or trends, such as excessive crying or sleep difficulties, that indicate mental health risks. This allows practitioners to make better-informed decisions. In this sense, AI augments human intelligence, improving the accuracy and comprehensiveness of client assessments.

\begin{quote}
    % \textit{"I can bring this [question] to my supervisee... [and get] five more questions back that I can ask."} (C1)

    \textit{"Not just you train the model, the model also trains them."} (S6)
\end{quote}

HAI collaboration also creates \textit{learning} opportunities for SSPs, especially junior personnel. S4 said the thorough examples generated by the model were "really helpful in... guiding the worker" to develop interventions and "expand their perspectives". S6 felt that AI could "train" workers as they used it, "polishing" them as caseworkers.

\begin{quote}
    % \textit{"I can bring this [question] to my supervisee... [and get] five more questions back that I can ask."} (C1)

    \textit{"And this can also be used in supervision! You know!"} (C1)
\end{quote}

Finally, we discovered the unexpected role of \textit{supervision} that AI can assist with. C1 pointing out how many of the AI's outputs, while not designed for that purpose, provided useful starting points for discussion and reflection with supervisees. S4 and S7 agreed, pointing out that the AI's ability to quickly "concretise theoretical models" to build on during sessions. W4 and W5 said the AI provided useful intervention suggestions for supervisees to bring into sessions. W9 even cited AI as a "readily-available supervisor". 

% AI provided useful prompts for discussion plays a valuable role in human-human-AI collaboration, especially in supervisory contexts. C1, a senior counsellor, explained how AI can assist in supervision sessions by providing a foundation for discussion and reflection. While AI-generated outputs might not be immediately applicable to experienced practitioners, they can serve as useful tools to guide less experienced workers. Supervisors can leverage AI outputs to facilitate discussions with their supervisees about potential intervention plans, creating a more robust and collaborative learning environment.
% These findings highlight the dynamic and multifaceted nature of human-AI collaboration in social work, where AI tools not only augment human capabilities but also foster new ways of working and learning in a collaborative environment.

% Another useful application of AI was its ability to be used in \textbf{human-human-AI settings} such as supervision. Extending the above quote, workers with differing levels of experience and positions may benefit from AI differently. C1, a senior counsellor, said: "at my level [this output] is not helpful [for my own work] because I know what to do already", but for supervision, "this I can bring... to see if my supervisee has used these questions [to ask the client], and if they haven't, I may want to introduce them". AI here provides a foundation on which C1 could build upon to more effectively facilitate a supervision session. Junior workers also expressed similar sentiments: when S4 brought up the tool's ability to quickly generate many different intervention plans, W4 said they "might not have thought of [some of these] interventions", and while he might not adopt them directly, he could discuss these with his supervisor on which ones to try out. This is an interesting sentiment, which surfaces the potential of not just human-to-AI collaboration, but also more complex dynamics involving more than two parties like human-human-AI collaboration and cooperation \cite{munyaka2023decision}. In the context of social service and the examples raised by our participants, we can see that AI can be employed by supervisors and junior workers as a facilitation tool for supervision sessions, allowing supervisor and supervisee to work collaboratively not just with one another, but also with AI, to develop and discuss different ideas such as intervention plans. Most human activities today are done collaboratively, and social service is no exception, where traditionally, senior SSPs serve as mentors to supervise and guide junior workers. When we add AI into the mix, AI tools can therefore serve as a de facto supervisor to similarly guide workers (especially those in more junior roles) and assist with and augment the human supervisor's role.

% Participants highlighted the potential of working with AI to facilitate client assessments.
% There has been emerging interest in HAI collaboration \cite{wang_human-human_2020}, a term that refers to the process in which teams, comprising of human and AI agents, "work together in a synergistic manner to achieve shared goals, e.g., with the AI providing recommendations or insights, and humans guiding and refining the AI-generated outputs" \cite{hemmer2024complementarity}. 
% A key way in which HAI collaboration could help in social service is to provide \textbf{HAI augmented intelligence in client assessments and diagnosis}. As the above quote by D1 reveals, SSPs may sometimes miss out on certain symptoms or signs that clients display (an understandable issue, given the lack of time and multiple demands that SSPs face). AI can help by recognising patterns or trends (e.g., excessive crying, difficulty sleeping) as potential mental health risks, thus bringing them to the attention of the SSP who can then make a better, more informed diagnosis of the case. In this sense, AI can augment the intelligence of humans by picking up on non-obvious patterns that social workers may miss out on or overlook, thereby increasing the accuracy of client assessments and subsequent interventions. This thus gives rise to a form of "augmented intelligence" \cite{jarrahi_artificial_2018}, whereby humans and AI can work together to enhance one another's intelligence and abilities beyond what an AI tool or a human worker alone could achieve on their own.

% Participants also cited the \textbf{benefits of HAI symbiosis in mutually learning from and training one another}. S6, a senior supervisor, noted that for junior workers who were new to the field and using AI to generate ideas, 
% \begin{quote}
%     \textit{"when they look at it, they will know that, oh, so this is how, the way that I should actually do it. And in terms, the more that when they do with the model helping them, and of course they will have to also put in their own effort to, you know get supervision from the supervisors and all these things, their knowledge, I think it will polish them as well. Not just you train the model, the model also train them. I think it works both ways."}
% \end{quote}
% This quote showcases the concept of HAI augmentation, whereby at the same time as the human worker trains and improves the AI, the AI simultaneously also helps to train and enhance the worker's skill, highlighting the duality and dynamic nature of HAI collaboration in social service.



% Our final theme highlights the importance of viewing AI through the dual lenses of \textit{collaboration}. Human-AI (HAI) collaboration has been extensively studied \textit{[Cite]} as new ways of improving human productivity and work processes; simultaneously, overlooking the need for collaboration when using AI tools can lead to many potential risks. We examine our findings from both of these angles. 

% First, we discuss the risks of a lack of collaboration. This is most salient in applications of instructions and guidance. The use of AI for ideation and session planning, despite its flaws, has been an omnipresent suggestion (e.g. S4, S6, W7, W11, W12, D1). However, its effectiveness here depends on the worker's individual competencies: a newer worker might be unable to compensate for the tool's shortcomings.
% In particular, the tension between the extensive theoretical underpinnings of social work and the realities of its dynamic and fast-changing nature create unique challenges.
%S9 used the example of a Task-Centered intervention suggested by the tool: 
%"So the step one, two, three means what? It means that I need to do it in the sequence, isn't it? So if you don't tell me and I'm a newbie, I’m thinking also, I need to do step one first and then step two and then step three and step four.

%"For our interventions, the safety plan is always the thing to prioritize. But it seems like [safety here is] at step four... and our interventions are not so linear, sometimes you make two steps forward, then you backtrack one time. So it depends on your target group. If newbies see this, I need to follow one, two, three, four steps, die \textit{liao}\footnote{A local slang term expressing resolution and finality.}."

%In essence, the intervention plan generated by the tool followed a theoretically-grounded sequence of steps, 
% These steps provide a useful reference for more experienced workers, but S9 pointed out that a newer worker would interpret it more 
%that when interpreted literally and rigidly produce a poor outcome. \textit{[Cite more here...]} The output, then, is a useful reference, but without either \textbf{human input by the worker to complement the system's guidance or more experienced workers to lend their expertise}, users can easily be led astray in the execution of their work.

%On the flip side, the same procedural, systematic nature of AI can also be a boon for human-AI collaboration. 

% Move this to discussion section?: What differentiates the social work field in how it has to be treated differently is...
% 

\subsection{Attitudes}

The values in Section \ref{subsec:ethos} give rise to three attitude themes along a spectrum of valence: \textbf{A}cceptance, \textbf{A}mbivalence, and \textbf{A}pprehension. These capture the widely varying feelings that SSPs hold toward AI. 
% \textbf{Apprehension} captures the negative or wary feelings of social workers towards AI, a largely unfamiliar and still-untested technology. \textbf{Acceptance} encapsulates the openness and optimism that social workers feel towards embracing and acceptance AI, along with its limitless possibilities. \textbf{Ambivalence} falls in the middle, with our participants demonstrating varying degrees of understanding towards AI and expressing a range of opinions about the extent to which AI can truly help in their work.

\subsubsection{Acceptance: Openness and Amazement}

Throughout our sessions, participants displayed a range of positive emotions towards AI.

\begin{quote}
    \textit{"This model is not perfect... But for it to continue to evolve further, there must be a willingness to try and to start moving things along... If it's here to stay, how can we make the best out of it?"} (D1)
\end{quote}

Participants expressed \textit{openness and curiosity} towards AI and its possibilities. D1 was "excited" by the potential benefits AI could bring to the sector, acknowledging its limitations but embracing the opportunity to incorporate it into practice. W5 noted, “There’s no harm in using something that makes your life easier,” and S4  highlighted the benefit of "expanding [workers'] perspectives".

% Extending from this sense of openness and acceptance, participants' \textit{amazement towards AI's capabilities} was also a contributory factor towards their positive sentiments towards it. There was a feeling of great astonishment, wonder, and even awe as participants discovered the algorithmic system's ability to summarize years' worth of case notes at a touch of a button (S6), infer client identities from shorthand notation (W3), and recognize acronyms for local organizations (S2). 

\begin{quote}
    \textit{"Let's see if it can pick up the strengths... oh, wow! Impressed."} (W5)
\end{quote}

Participants were also \textit{amazed by AI’s capabilities}, such as its ability to summarize years of case notes, infer client identities from shorthand, and recognize local acronyms. W3, for example, marveled at how AI inferred “DG” as “daughter” without context: “Oh my god... they know that A is the daughter.” Similarly, S2 was impressed by AI’s inference of “SYC” as Syariah Court, automatically generating relevant legal advice. [add more here and a conclusion, and we're good!]

% Participants were impressed by how the system could infer names (W3) and institutions (S2) from shorthand or initialisms.
% In one instance, W3, a SSP who was testing out the tool by inputting his own case notes from a session with a client, remarked in amazement, 

% \begin{quote}
%     \textit{"Oh my god, I didn't even mention that it's a daughter, right? They know that DG is daughter. I put DG, then I put A...Then they [the AI] know that A is the daughter. 'Ensuring her daughter (A).'"}
% \end{quote}

% His exclamation of surprise reveals his astonishment at AI's ability to intelligently infer and accurately guess the identity and relationship between his client and daughter A, without any context or explanation of the abbreviation "DG" that he used in place of the word "daughter". Similarly, on another occasion, S2 also found himself amazed by the capability of AI to make intelligent inferences from his raw notes:

% \begin{quote}
%     \textit{"They [AI] can actually pull out data because I indicated SYC [Syariah Court], so they already know how to link it up with legal advice. It's quite good. SYC is for divorce. They were able to retrieve it and put it in the component for legal advice, which is relevant."}
% \end{quote}

% Despite him not explicitly referring to the acronym "SYC" as "Syariah Court" (a Muslim institution in charge of settling disputes between divorcing parties), S2 was impressed by the AI tool's ability to infer the organisation and automatically generate appropriate recommendations for legal advice for the client, which he felt was "relevant" and "good". Therefore, overall, from participants' responses, we can see that SSPs in general were impressed and amazed by AI's abilities, and open-minded in trying out different ways in which they could utilise the algorithmic system enhance their existing work practices, such as in summarising case notes and generating client recommendations with greater ease.

% Some participants frequently expressed amazement at the AI's capabilities. "Oh my god," said S6 at the possibility of summarizing years' worth of case notes with the click of a button. W3 was similarly impressed by the LLM's intelligence: "Oh my god, I didn't even mention that it's a daughter, right? They know that DG is daughter. I put DG, then I put A. Someone is like DG, then bracket A. Then they know that A is the daughter. No, you see? Ensuring her daughter, bracket A." S2 was amazed at how "they can actually pull out data, because I indicated SYC [Syariah Court; an acronym for a local organisation], so they already know how to link it up with legal advice," liking the system's ability to understand local terms and subsequently draw inferences from it.

% Notably, many participants were willing to embrace AI despite its flaws. For example, when the system gave an overly verbose output, S2 and S3 adapted by "just... sift[ing] through the info" and pick[ing] out what is relevant", and W2 said that it still reduced their mental effort in formulating the case. In another case, W1 had the system misinterpret an individual mentioned in their input, but said, "Yeah, but I mean I think... I would just [use it], then amend if I need to amend".

% Also include amazement >> product of their proficiencies, what's lacking there, how this leads to amazement

\subsubsection{Apprehension: Distrust of AI}
\label{subsubsec:apprehension}

Despite their positive attitude towards AI, SSPs also expressed exhibited apprehension regarding the risks and limitations of algorithmic systems. 
% Here, we can see how the ethos and principles of SSPs (Section \ref{subsubsec:ethics}) inform and contribute towards their attitudes about AI. 

\begin{quote}
    \textit{"I would say right now, we are prepared to be more cautious."} (D1)
\end{quote}

A major concern was the \textit{tension between the highly confidential nature of social work data and the opacity of third-party AI systems}, coupled with the nascent nature of generative AI. D1 considered it a "very gray" area in which he was "prepared to... be more cautious". Echoing their ethos of protecting client privacy
% Firstly, participants were notably \textit{concerned about the black box nature and nascence of AI systems}. AI has often been criticised for its opacity and lack of transparency, essentially serving as a "black box" \cite{castelvecchi2016can} that can be difficult for people, especially non-technical experts, to understand. The black box nature of AI systems developed by multinational corporations (which themselves often have a lack of transparency on data management policies and protocols), the highly confidential and sensitive nature of social service work, and the nascence and novelty of AI and LLMs in the field therefore give rise to significant worries in adopting AI in the social sector and make it a "very gray" area for SSPs to navigate (D1). In particular, echoing their ethos of protecting client privacy 
(Section \ref{subsubsec:ethics}), many workers were concerned about entering (W5, W8) and storing (S1) client information into an external server, and even about the security of the AI system itself (S7). Both third-party data storage and the process of feeding client data to an AI model (i.e. an LLM) were causes for concern.
% These fears and concerns about the lack of transparency and inability of AI to properly safeguard client safety and privacy therefore contribute towards a sense of apprehension, distrust and hesitance towards fully embracing AI in the social work practice.

% ?Therefore, we can see how in spite of their aforementioned positivity and acknowledgement of AI's beneficial capabilities, SSPs nonetheless still have their reservations and apprehension towards AI, and are hesitant towards fully embracing it in social service due to privacy and safety risk concerns. This is an important element for designers to remember as they design AI systems for social service (or any field in general): a technology can have many irrefutable benefits, but designers always have to keep in mind the attitudes and core principles of users when designing a tool in order to overcome their fears and reservations. Specifically, in the case of social service, due to the importance of ethical principles and sensitivity of the work of SSPs, \textbf{it is essential for designers to develop AI tools that can safeguard the safety and privacy of clients and offer greater transparency}, so as to truly convince and convert practitioners to adopt and utilise AI.
% W5 talked about needing to create and "set a common protocol".

% The center director D1 said: "It's in our code of ethics..., so we want to protect as much as we can... Right now if you ask me, we are prepared to say, to be more cautious." Yet, in requesting participants to only "delete \textit{some} of this private information", it is clear how the use of AI is largely a "very grey" area that warrants significant consideration.

% Another concern was \textit{the inability of AI to handle the nuances} of social work. The irreplaceable experience of SSPs (Section \ref{subsubsec:experience}) led to sentiments of AI inadequacy in certain areas, 

% S4 expressed confusion over the AI's output: "I don't know why [the AI] gave me this." W5 was more circumspect, saying, "how can the model [do this]? I think that one is hard." 
% reveals, the experience and expertise of SSPs, which imparts them with a human touch and ability to understand the dynamic context of their clients' cases and circumstances, are important and irreplaceable parts of the social service practice. In implementing an AI tool, participants were therefore naturally concerned and apprehensive about the machine's ability to adequately replicate the human experience and grasp these subtle nuances. In one example, S4 had some reservations about the algorithmically generated output when testing the AI tool to come up with recommendations for an actual case he had involving a father and son:
% SSPs questioned AI’s ability to grasp the nuances of social work. Social service practice often requires a "human touch" to evaluate complex client contexts, something participants felt AI struggled with. 
% \begin{quote}
%     \textit{"This is SFBT...SFBT wasn't used [with the actual client] because simply the person wasn't ready to engage. So there is no subsequent moving on for this case. Like some examples may not be contextual, like 'considering your strong support'. I don't know why they [the AI] gave me this. [Or] 'How have you and your friends helped you cope with the marital distance and parenting challenges?' I guess for the dad, there wasn't any really real issues for his coping. So I think we would have covered that, really, in terms of how his friends helped him.}
% \end{quote}
% S4 mentioned how the AI system suggested using SFBT, but missed how "the person wasn't ready to engage. So there is no subsequent moving on for this case."
% As the quote reveals, AI can have certain limitations in grasping the nuances and contexts of a case, which human SSPs can more readily pick up on. 
% In the above case, the AI system recommended a SFBT intervention for the client, which S4 judged as inappropriate as "the person wasn't ready to engage", showing how unlike the AI, the SSP was able to evaluate the suitability of intervention modes and approaches based on the client's state of mind and circumstances. This is an important dimension of social work practice, which is so highly individualistic and specific to clients' differing and dynamic situations that it requires the human expertise of a human worker to judge and recommend measures that are tailored to the client's needs, which an algorithm may not be able to accomplish. Similarly, the AI generated a question asking the client about how his friends helped with coping with marital and parenting challenges, which S4 again judged as inappropriate and irrelevant, given that the client did not face any coping issues. Therefore, while the AI may have superior information and data processing capabilities, we can see here that the human expertise and experience in evaluating the client's individual needs are ultimately still superior to the machine. 
% W5 raised questions about cases that were "already open for quite a while... I don't know how the model can actually help that... how can the model actually also list down the progress? I think that one is hard." 

% Therefore. the inadequacy of AI to accurately capture and comprehend the complex nuances involved in social service contribute towards SSPs' reservations and apprehension towards fully utilising them in their practice. 

% This emphasises to us that even while we try to implement AI in social service, there is still an irrefutable human dimension that cannot be easily outsourced or replaced, making it vital for us to \textit{complement the capabilities of machine and man in social practice}.

% Principles > distrust that AI can really d handle their issues

% This links to the issue of human perception and the core role it plays in 

% Perception > Distrust: Wary that AI cannot capture some capabilities of humans

\begin{quote}
    \textit{"One of our concerns is... [will using this AI] actually disable our ability to make assessment?"} (D1)
\end{quote}

There were also \textit{concerns over overuse and overreliance on AI}.
% worrying that the overuse and outsourcing of tasks to AI may lead to over-dependence and even degradation of ability for SSPs to perform tasks on their own. In the quote highlighted at the top of this section, the center director, 
These centered around the possibility of degradation of SSP's skills and judgement (D1). 
% D1, raised their primary concerns on the adoption of AI, citing worries that it may weaken human workers' ability to exercise their own judgment in decision-making and assessments. In another session, D1 also noted that: 
% \begin{quote}
%     \textit{"Some of our colleagues have...raised a concern about [AI] that then if we move forward with this, then [it may] impair the social workers' ability to make assessment. Because...if you find that it is useful, then the more you use it, then the more you rely on it, then you stop using your own."}
% \end{quote}
S3 agreed about the risk of overrliance by "spoonfeeding" junior workers, and S9 noted the need for workers to "still use their brain... otherwise... they just rely on this."
S9 also worried about how junior workers might fail to recognise suboptimal outputs by AI, and be misled as a result.
% His sentiments are mirrored by S3, a senior supervisor, who agreed that, "there will be a reliance on it if it is given spoon-fed to them...they will be reliant on this." The above quotes reveal the double-edged nature of AI's efficacy. While on one hand, it can offer clear benefits to helping SSPs to improve the speed and accuracy of their assessments and reporting. However, on the other hand, the usefulness of AI can also make it easy for it to become a handicap and a crutch, whereby human workers end up using it more and more, at the expense of their own decision-making skills. As supervisor S9 highlighted, "I think the expectation need[s] to be very clearly communicated. This [AI] is to help you with documentation. But your case conceptualization still need to use your brain. Right? Otherwise, I think our new colleagues just slowly rely on this." There is thus a very valid fear that the overuse and overdependence on AI over time can lead to a deterioration of workers' skill and threaten their agency and autonomy in making decisions for themselves.

\subsubsection{Ambivalence: Uncertainty and Conflicting Sentiments}

Finally, we present the intersection between embracing AI and rejecting it: the \textit{ambivalance} of intra- and inter-personal conflict in viewpoints and feelings towards AI.
% because participants not only displayed an awareness of the limitations of technology, but were also willing to find ways to work around and with it to harness its benefits while respecting its limits.
% For instance, some participants discussed the tendency of the system to output generic or overly verbose text. 
% For instance, many participants S6 analyzed the system's output: "It also depends on how accurate the case notes we put in are, because I put in a very generic one, then it just analyzes it accordingly and then you just give me a very generic form of interventions... So that means if you want to have an accurate kind of very precise intervention, then the way that we actually write it, you have to feed it as much info as possible." 
% S3 discussed how they would use a report generated by the system: "You cannot just copy blindly. You must choose, pick and choose which one is relevant to your case, and then put it up accordingly." Similarly, S2 commented that "You just have to sift through the info and pick out what is relevant in different areas." W2 said, "I feel that sometimes it's that they will give... I think it's more like the \textit{duh}\footnote{A local slang term meaning obvious and not worth much further thought.} information like you mentioned that sometimes I have to read and then I don't think that is as relevant. So I will just not use it. But I think it's okay. The time that it takes is more like I'm just reading.
% I'm not actually having to go and think so much, \textit{How do I want to formulate this}? So I just need to read and then if it's helpful, then I will just put it in." Another participant tried a set of case notes where the client colloquially referred to her boss as "uncle", causing the system to misinterpret the individuals involved in the case: "Yeah, but I mean this I think is just... I have to correct it. I would just copy and paste on my assessment. Then I amend if I need to amend." These participants all noted how the AI system, given limited input or context to work with, failed to give the most concise or suitable outputs; yet at the same time, they demonstrated a willingness to adapt their work patterns to harness the benefits it provided.

\begin{quote}
    \textit{"Efficiency-wise, I'm really still on the fence, because I'm spending time giving prompts to the [AI]."} (S4)
\end{quote}

% A few participants were unsure about the benefits of AI.

% \begin{quote}
%     \textit{"All seem relevant, but I'm not sure which one to specifically pick up?"} (W11)
% \end{quote}

Participants were sometimes \textit{unsure if they would benefit from an AI system}, weighing if the benefits of a mostly-accurate AI system outweighed the effort of using it. Examples of such outputs included case recordings that might miss out on specific details (S2, W11), sample interventions that lacked specificity (S4), and reports that might turn out too lengthy and require trimming (S5). A related sentiment came up discussing potential future ideas, specifically with use cases that required a large model context window: S6 and W5 "didn't know" how useful a summarisation tool for years' of past reports would be. 
% This possibly hinted at an incoherence between their mental models of technological capabilities and the state of modern LLMs.


\begin{quote}
    \textit{"It's not very nice when, you know, people talk to me... [and I'm like] keep tap tap tap [on the laptop].} (S6)
\end{quote}


\textit{Usage of technology in the presence of a client} was also a contentious topic, given the discussions on using AI systems during client sessions. S2 was "not comfortable" using a laptop while attending directly to a client, but W1 was.
% D1 was happy to audio-record sessions for real-time processing by the AI. 
S6 and W5 disliked live note-taking on a laptop, but were happy to replace it by audio recording the sessions.

% S10 discussed an assessment produced by the system: "So because this one, I mean AI also has certain limitations... So I think that what is for us to actually emphasize with the supervisee that these are just guidelines, but you also need to customize it based on where your client is at and where you are at in terms of your experience and confidence. So that's my thought." This demonstrated an additional element of involving not just a single user, but multiple stakeholders in adapting to the introduction of AI technologies in their daily work.


\begin{quote}
    \textit{"It's the supervisor's role to keep emphasising to the supervisee: to not be married to this assessment."} (S10)
\end{quote}

Finally, participants were divided over the 
% potential of overreliance 
\textit{potential negative effects on worker skills} of AI. S7 felt face-to-face client interactions were still the litmus test of a worker's skill: "it will eventually be clear that this was the recommendation of [the tool] but then you went and did something else... and then you'll see that it's just a mess in that way." S3 agreed: "When they do their work, it is mostly real-time. You don't go back to pen and paper and start to develop [a solution], but it's more about what is presented to them immediately [and how they react]."
% S5 felt it unlikely that workers would "bring the[ir] laptops in" and directly read off the screen to their clients. 
% These participants indicated that the human nature of the social work profession itself guarded against overreliance on computer systems. 
On the other hand, others still expressed caution. S9 felt "the expectation [for use] needs to be very clearly communicated", and S10 wanted "to actually emphasize with the supervisee that these are just guidelines" rather than a gospel to be followed. S7 mentioned the "integrity of their work", hinting at a need for workers to maintain an awareness that the system was only an aid and not a replacement for their skills.

% The above examples showcase some key points of uncertainty about how AI and technology fit into the sector; undoubtedly, these are some of the most important questions going forward. 

% mention quote on precedence?

% Yet, the use of AI here presents an ethical conundrum. Participants mentioned multiple times how risk and safety concerns (i.e. any potential threats to the physical safety of the client)
% Yet, herein lies the ethical conundrum of utilizing AI in social work: it can help social workers to reduce the mental and manual burdens of data cleaning and processing, but before doing so, they need to first and foremost ensure that it is in line with "

% These statements show that social workers recognize and value the tremendous time-saving benefits that AI can offer, but are hesitant and cautious about using them due to potential privacy concerns (e.g., whether the AI tool would retain clients' information, or whether the data would be used to train the AI model). , and with the technological advancements and accelerated data processing powers brought about by big data and AI technologies, "[t]oday's social workers face issues involving values and ethics that their predecessors in the profession could not possibly have imagined", including concerns of monitoring, surveillance, data privacy and confidentiality \cite{reamer2018social}. Our interviews therefore underscore the importance of data privacy as a core value of social workers and the exigency of designing and developing ethical AI systems that can safeguard and protect the confidentiality and personal information of clients in the context of social work.


% Proficiency >> accepting how AI can "replace" some part of their work
% i just briefly go through these sections and feel the quotes and illustrations are good. But how can i connect them with 5.2.1 and 5.2.2? I feel 5.2.1/2 is the main question that we want to answer, so we may need to correspond our findings to them explicitly?

==> sections-old/7_discussion.tex <==

\section{Discussion}

% \begin{quote}
% \textit{"We believe it is unethical for social workers not to learn... about technology-mediated social work."} (\citeauthor{singer_ai_2023}, 2023)
% \end{quote}

In this paper, we raise a number of formative insights on the use of generative AI in the social service sector. In this section, we briefly recap our main findings from our PD studies, before discussing theoretical implications and design suggestions.

\subsection{Uses and Risks of AI in the Social Service Sector}
%MH: is this section for summarizing the results?

Returning to the overall question of the role and place of AI in the social sector, we refer to the research areas identified in Sections \ref{sec:stage2designuses} and \ref{sec:stage2designrisks}. 

\subsubsection{Uses of AI} 
\label{subsubsec:discussionuses}

We uncovered multiple potential uses of AI, both obvious and not-so-obvious. Participants found many applications of generative AI in assisting with the multiple writing-focused tasks in the social service sector, such as summarising intake information, formatting case recordings, and report writing. Participants generally were happy to embrace AI for such tasks, even when the system made occasional errors (e.g. misinterpreting a nickname given by the worker to the client) or was not fully calibrated (e.g. giving overly lengthy outputs); many indicated a willingness to work around these errors and make manual corrections where needed.

Participants also found many uses for AI to help with cognitively challenging tasks, but had more mixed evaluations of the system's outputs here. Evaluations of the client according to various theories and metrics of social work were deemed somewhat useful; participants noted that while they might not use the output directly, it still served as a good starting point from which to work and provided learning points for even more experienced workers. With the proposed interventions, the workers similarly found these to provide inspiration and ideas, although they would not adopt them directly for use.

One unexpected use of AI that emerged prominently was as a supervisory aid. Our participants mainly described supervision sessions as senior and junior workers discussing how to formulate and proceed with a case further. With this, the suggested interventions or possible solutions generated by our AI system served as good discussion points. 

\subsubsection{Risks of AI}
\label{subsubsec:discussionrisks}

We also found multiple areas where participants identified risks in using AI. Most of these related to misleading, if not technically incorrect, outputs from the system potentially leading workers to inappropriate solutions with clients. These outputs included an insufficient focus on client risk and safety and overly rigid intervention plans. These concerns were mostly raised by supervisors and senior workers, who noted the importance of active discussion between supervisor and supervisee to go over the AI's suggested course of action. Senior staff also mentioned the risk of overreliance on AI, although they were generally less concerned about this due to the constant engagement of workers with both their client and supervisors.

\subsection{Overcoming Negative Effects of Introducing AI}
\label{subsubsec:discussionnegative}

Past work has shown that the introduction of AI can disrupt practitioners' workflows, both in social work \cite{kawakami2022improving} and adjacent fields \cite{elwyn2013many}; this reduces their usage and effectiveness and creates negative or indifferent attitudes towards AI \cite{de2020case, brown2019toward}, In our study, however, participants generally seemed welcoming to our generative AI system, being happy to suggest and discuss new features while bringing in examples from their own work. We suggest some differences that make generative AI in the social service sector different in this regard. First, their greater outcome-to-effort ratio makes them a more attractive prospect. The social service field involves a large amount of verbose evaluation, something which suits the strengths of LLMs. Second, the inherent uncertainty and variation in cases that SSPs encounter means that correctly assessing how to serve a client can be a daunting task, especially for newer workers. The adaptability and wide knowledge base of LLM-based AI systems serves as a welcome aid for workers looking for ways to conceptualise and understand a case, rather than the system simply recommending actions for workers to take.
% MH: i do not fully understand the relation between 'outcome-to-effort ratio' and verbose evaluation/ai aid
% "adaptability and wide knowledge base" do we need to cite here

This points to an important consideration for how AI systems could be implemented in the social sector. There are many areas in which SSPs face high workloads. AI systems can therefore be positioned as a way to reduce these workloads, rather than as a substitute for human decision making.
% MH: what is the relation between this paragraph and the last one? I feel they are talking similar things

Of course, past work \cite{yang2019unremarkable, kawakami2022improving} highlights the difficulty of implementing AI systems in real workplaces, with workers rejecting them for a variety of reasons. 
% how many AI systems fail  past AI systems "performed well in the lab" but failed in the real world;
Our "in the lab" study similarly is not guaranteed a successful transition. We suggest, however, that most of these failings pertained not to actual system design or interface, but rather how it fit into the broader landscape of the user's work (see Sections \ref{subsec:relatedworkaiuse}). We tackle these issues by integrating them directly into our FGD design: the very motive of the FGDs was to understand how workers would use the system in their daily lives. In this, we address the concerns raised in previous studies: in sitting down with case workers and having them use our system as though they were processing case data, we were able to simulate their real working environment in a way unfeasible for studies dealing with call centres or operating theatres. We therefore suggest that our findings are more likely to translate to real use. 
% MH: what is the relation between this and 'Overcoming negative effects of introducing AI'..?



\subsection{Embracing Imperfect AI}
\label{subsec:discussionimperfectai}

Our findings address the call to understand \textit{"how collaborative decision-making [...] impacts how people rely upon and make sense of AI models"} \cite{kawakami2022improving}. As with many past studies \cite{kawakami2022improving, yang2019unremarkable, saxena2021framework}, our users highlighted many areas where the AI's output was inadequate for direct use. 
% Clearly, there were many areas in which users could not directly "rely upon" the inadequate output of the AI. 
We do not elucidate and analyse these specific flaws, since these may be specific to GPT-4. Rather, with the assumption that AI will never be perfect, we are interested in how the \textit{very presence of inadequacies affects the way users interact with the system}. 
% Here is where collaboration, both human-with-human and human-with-AI, come to the fore.

What was noteworthy to us was that any time a participant criticised the system's output as inadequate, they often followed up with: \textit{so this is something the supervisor must emphasise to the junior worker}. Rather than filtering out less useful AI features, our participants constantly - and without prompting - discussed how they might be used in collaborative efforts. Section \ref{subsubsec:collaboration} showed many such instances; C1, in particular, hinted at how AI inadvertently helped her see the perspective of a junior worker, by virtue of giving less complete outputs; this served as a basis for supervision. Clearly, present AI is not a perfect substitute for human experience and expertise. However, even this imperfect AI became a starting point for brainstorming more complete interventions or discussions between workers about a case formulation. 

% The strong, inherent element of collaboration and constant communication that takes place in Agency A thus seems to provide a good fit for generative AI systems: AI plays the role of \textit{facilitating} discussions and learning amongst workers of the agency.

The idea of embracing imperfect AI echoes the findings of \citeauthor{bossen2023batman} (2023) in a clinical decision setting, which examined the successful implementation of an "error-prone but useful AI tool". This study frames human-AI collaboration as "Batman and Robin", where AI is a useful but ultimately less skilled sidekick that plays second fiddle to Batman. This is similar to \citeauthor{yang2019unremarkable}'s (2019) idea of "unremarkable AI", systems designed to be unobtrusive and only visible to the user when they add some value. As compared to \citeauthor{bossen2023batman}, however, we see fewer instances of our AI system producing errors, and more examples of it providing learning and collaborative opportunities and other new use cases. We build on the idea of "complementary performance" \cite{bansal2021does}, which discusses how the unique expertise of AI enhances human decision-making performance beyond what humans can achieve alone. Beyond decision-making, generative AI can now enable "complementary work patterns", where the nature of its outputs enables humans to carry out their work in entirely new ways. Our study suggests that rather being a sidekick - Robin - AI is growing into the role of a "second Batman" or "AI-Batman": an entity with distinct abilities and expertise from humans, and that contributes in its own unique way. There is certainly still a time and place for unremarkable AI, but exploring uses beyond that paradigm uncovers entirely new areas of system design.

% \cite{gero2022sparks} found AI to be useful for science writers to translate ideas already in their head into words, and to provide new perspectives to spark further inspiration. \textit{But how is ours different from theirs?}

\subsection{New Avenues of Human-AI Collaboration}
\label{subsubsec:discussionhaicollaboration}

Past HCI literature in other areas \cite{nah2023generative} has suggested that generative AI represents a "leap" \cite{singh2023hide} in human-AI collaboration, 
% Even when an AI system sometimes produces irrelevant outputs, it can still provide users 
% Such systems have been proposed as ways to 
helping users discover new viewpoints \cite{singh2023hide}, scour existing literature to suggest new hypotheses 
\cite{cascella2023evaluating} and answer questions \cite{biswas2023role}, stimulate their cognitive processes \cite{memmert2023towards}, and overcome "writer's block" \cite{singh2023hide, cooper2023examining} (particularly relevant to SSPs and the vast amount of writing required of them). Our study finds promise for AI to help SSPs in all of these areas. By nature of being more verbose and capable of generating large amounts of content, generative AI seems to create a new way in which AI can complement human work and expertise. Our system, as LLMs tend to do, produced a lot of "bullshit" (S6) \cite{frankfurt2005bullshit} - superficially true statements that were often only "tangentially related" and "devoid of meaning" \cite{halloran2023ai}. Yet, many participants cited the page-long analyses and detailed multi-step intervention plans generated by the AI system to be a good starting point for further discussion, both to better conceptualize a particular case and to facilitate general worker growth and development. Almost like throwing mud at a wall to see what sticks, generative AI can quickly produce a long list of ideas or information, before the worker glances through it and quickly identifies the more interesting points to discuss. Playing the proposed role as a "scaffold" for further work \cite{cooper2023examining}, generative AI, literally, generates new opportunities for novel and more effective processes and perspectives that previous systems (e.g., PRMs) could not. This represents an entirely new mode of human-AI collaboration.
% This represents a new mode of collaboration not possible with the largely quantitative AI models (like PRMs) of the past.

Our work therefore supports and extends prior research that have postulated the the potential of AI's shifting roles from decision-maker to human-supporter \cite{wang_human-human_2020}. \citeauthor{siemon2022elaborating} (2022) suggests the role of AI as a "creator" or "coordinator", rather than merely providing "process guidance" \cite{memmert2023towards} that does not contribute to brainstorming. Similarly, \citeauthor{memmert2023towards} (2023) propose generative AI as a step forward from providing meta-level process guidance (i.e. facilitating user tasks) to actively contributing content and aiding brainstorming. We suggest that beyond content-support, AI can even create new work processes that were not possible without generative AI. In this sense, AI has come full circle, becoming a "meta-facilitator".

% --- WIP BELOW ---

% Our work echoes and extends previous research on HAI collaboration in tasks requiring a human touch. \cite{gero2023social} found AI to be a safe space for creative writers to bounce ideas off of and document their inner thoughts. \cite{dhillon2024shaping} reference the idea of appropriate scaffolding in argumentative writing, where the user is providing with guidance appropriate for their competency level, and also warns of decreased satisfaction and ownership from AI use. 

Separately, we draw parallels with the field of creative writing, where HAI collaboration has been extensively researched. Writers note the "irreducibly human" aspect of creativity in writing \cite{gero2023social}, similar to the "human touch" core to social service practice (D1); both groups therefore expressed few concerns about AI taking over core aspects of their jobs. Another interesting parallel was how writers often appreciated the "uncertainty" \cite{wan2024felt} and "randomness" \cite{clark2018creative} of AI systems, which served as a source of inspiration. This echoes the idea of "imperfect AI" "expanding [the] perspective[s]" (S4) of our participants when they simply skimmed through what the AI produced. \cite{wan2024felt} cited how the "duality of uncertainty in the creativity process advances the exploration of the imperfection of generative AI models". While social service work is not typically regarded as "creative", practitioners nonetheless go through processes of ideation and iteration while formulating a case. Our study showed hints of how AI can help with various forms of ideation, but, drawing inspiration from creative writing tools, future studies could consider designs more explicitly geared towards creativity - for instance, by attempting to fit a given case into a number of different theories or modalities, and displaying them together for the user to consider. While many of these assessments may be imperfect or even downnright nonsensical, they may contain valuable ideas and new angles on viewing the case that the practitioner can integrate into their own assessment.

% \cite{foong2024designing}, describing the design of caregiver-facing values elicitation tools, cites the "twin scenarios" that caregivers face - private use, where they might use a tool to discover their patient's values, and collaborative use, where they discuss the resulting values with other parties close to the patient. This closely mirrors how SSPs in our study reference both individual and collaborative uses of our tool. Unlike in \cite{foong2024designing}, however, we do not see a resulting need to design a "staged approach" with distinct interface features for both stages.

% --- END OF WIP ---

Having mentioned algorithm aversion previously, we also make a quick point here on the other end of the spectrum - automation bias, or blind trust in an automated system \cite{brown2019toward}. LLMs risk being perceived as an "ultimate epistemic authority" \cite{cooper2023examining} due to their detailed, life-like outputs. While automation bias has been studied in many contexts, including in the social sector or adjacent areas, we suggest that the very nature of generative AI systems fundamentally inhibits automation bias. The tendency of generative AI to produce verbose, lengthy explanations prompts users to read and think through the machine's judgement before accepting it, bringing up opportunities to disagree with the machine's opinion. This guards against blind acceptance of the system's recommendations, particularly in the culture of a social work agency where constant dialogue - including discussing AI-produced work - is the norm.


% : Perception of AI in Social Service Work ??

\subsection{Redefining the Boundary}
\label{subsubsec:discussiontheoretical}

As \citeauthor{meilvang_working_2023} (2023) describes, the social service profession has sought to distance itself from comprising mostly "administrative work" \cite{abbott2016boundaries}, and workers have long tried to tried to reduce their considerable time \cite{socialraadgiverforening2010notat} spent on such tasks in favour of actual casework with clients \cite{toren1972social}. Our study, however, suggests a blurring of the line between "manual" administrative tasks and "mental" casework that draws on practitioner expertise. Many tasks our participants cited involve elements of both: for instance, documenting a case recording requires selecting only the relevant information to include, and planning an intervention can be an iterative process of drafting a plan and discussing it with colleagues and superiors. This all stems from the fact that generative AI can produce virtually any document required by the user, but this document almost always requires revision under a watchful human eye.

\citeauthor{meilvang_working_2023} (2023) also describes a more recent shift in the perceived accepted boundary of AI interventions in social service work. From "defending [the] jurisdiction [of social service work] against artificial intelligence" in the early days of PRM and other statistical assessment tools, the community has started to embrace AI as a "decision-support ... element in the assessment process". Our study concurs and frames generative AI as a source of information that can be used to support and qualify the assessments of SSPs \cite{meilvang_working_2023}, but suggests that we can take a step further: AI can be viewed as a \textit{facilitator} rather than just a supporter. Generative AI can facilitate a wide range of discussions that promote efficiency, encourage worker learning and growth, and ultimately enhance client outcomes. This entails a much larger scope of AI use, where practitioners use the information provided by AI in a range of new scenarios. 

Taken together, these suggest a new focus for boundary work and, more broadly, HCI research. GAI can play a role not just in menial documentation or decision-support, but can be deeply ingrained into every facet of the social service workflow to open new opportunities for worker growth, workflow optimisation, and ultimately improved client outcomes. Future research can therefore investigate the deeper, organisational-level effects of these new uses of AI, and their resulting impact on the role of profession discretion in effective social service work.

% MH: oh i feel this paragraph is quite new to me! Could we elaborate this more, and truncate the first two paragraphs a bit to adjust the word propotion?


% Our study extensively documents this for the first time in social service practice, and in the process reveals new insights about how AI can play such a role.



\subsection{Design Implications}

% Add link from ACE diagram?

% EJ: it would be interesting to discuss how LLMs could help "hands-on experience" in the discussion section

Addressing the struggle of integrating AI amidst the tension between machine assessment and expert judgement, we reframe AI as an \textit{facilitator} rather than an algorithm or decision-support tool, alleviating many concerns about trust and explainablity. We now present a high-level framework (Figure \ref{fig:hai-collaboration}) on human-AI collaboration, presenting a new perspective on designing effective AI systems that can be applied to both the social service sector and beyond.

\begin{figure}
    \centering
    \includegraphics[scale=0.15]{images/designframework.png}
    \caption{Framework for Human-AI Collaboration}
    \label{fig:hai-collaboration}
    \Description{An image showing our framework for Human-AI Collaboration. It shows that as stakeholder level increases from junior to senior, the directness of use shifts from co-creation to provision.}
\end{figure}
% MH: so this paradigm is proposed by us? I wonder if this could a part of results as well..?

% \subsubsection{From Creation to Provision}

In Section \ref{sec:stage2findings}, we uncovered the different ways in which SSPs of varying seniorities use, evaluate, and suggest uses of AI. These are intrinsically tied to the perspectives and levels of expertise that each stakeholder possesses. We therefore position the role of AI along the scale of \textit{creation} to \textit{provision}. 

With junior workers, we recommend \textbf{designing tools for co-creation}: systems that aid the least experienced workers in creating the required deliverables for their work. Rather than \textit{telling} workers what to do - a difficult task in any case given the complexity of social work solutions - AI systems should instead \textit{co-create} deliverables required of these workers. These encompass the multitude of use cases that junior workers found useful: creating reports, suggesting perspectives from which to formulate a case, and providing a starting template for possible intervention plans. Notably, since AI outputs are not perfect, we emphasise the "co" in "co-creation": AI should only be a part of the workflow that also includes active engagement on the part of the SSPs and proactive discussion with supervisors. 

For more experienced SSPs, we recommend \textbf{designing tools for provision}. Again, this is not the mere provision of recommendations or courses of action with clients, but rather that of resources which complement the needs of workers with greater responsibilities. This notably includes supplying materials to aid with supervision, a novel use case that to our knowledge has not surfaced in previous literature. In addition, senior workers also benefit greatly from manual tasks such as routine report writing and data processing. Since these workers are more experienced and can better spot inaccuracies in AI output, we suggest that AI can "provide" a more finished product that requires less vetting and corrections, and which can be used more directly as part of required deliverables.

% MH: can we seperate here? above is about the guidance to paradigm, below is the practical roadmap for implementation
In terms of concrete design features, given the constant focus on discussing AI outputs between colleagues in our FGDs, we recommend that AI tools, particularly those for junior workers, \textbf{include collaborative features} that facilitate feedback and idea sharing between users. We also suggest that designers work closely with domain experts (i.e. social work practitioners and agencies) to identify areas where the given AI model tends to make more mistakes, and to build in features that \textbf{highlight potential mistakes or inadequacies} in the AI's output to facilitate further discussion and avoid workers adopting suboptimal suggestions. 

We also point out a fundamental difference between generative AI systems and previous systems: that generative AI can now play an important role in aiding users \textit{regardless of its flaws}. The nature of generative AI means that it promotes discussion and opens up new workflows by nature of its verbose and potentially incomplete outputs. Rather than working towards more accurate or explainable outcomes, which may in any case have minimal improvement on worker outcomes \cite{li2024advanced}, designers can also focus on \textbf{understanding how generative AI outputs can augment existing user flows and create new ones}.

% for more senior workers...

% how to differentiate levels of workers?

% \subsubsection{Provider}

% The most basic and obvious role of modern AI that we identify leverages the main strength of LLMs. They have the ability to produce high-quality writing from short, point-form, or otherwise messy and disjoint case notes that user often have \textit{[cite participant here]}. 

Finally, given the limited expertise of many workers at using AI, it is important that systems \textbf{explicitly guide users to the features they need}, rather than simply relying on the ability of GAI to understand complex user instructions. For example, in the case of flexibility in use cases (Section \ref{subsubsec:control}), systems should include user flows that help combine multiple intervention and assessment modalities in order to directly meet the needs of workers.

\subsection{Limitations and Future Work}

While we attempt to mimic a contextual inquiry and work environment in our study design, there is no substitute for real data from actual system deployment. The use of an AI system in day-to-day work could reveal a different set of insights. Future studies could in particular study how the longitudinal context of how user attitudes, behaviours, preferences, and work outputs change with extended use of AI. 

While we tried to include practitioners from different agencies, roles, and seniorities, social service practice may differ culturally or procedurally in other agencies or countries. Future studies could investigate different kinds of social service agencies and in different cultures to see if AI is similarly useful there.

As the study was conducted in a country with relatively high technology literacy, participants naturally had a higher baseline understanding and acceptance of AI and other computer systems. However, we emphasise that our findings are not contingent on this - rather, we suggest that our proposed lens of viewing AI in the social sector is a means for engaging in relevant stakeholders and ensuring the effective design and implementation of AI in the social sector, regardless of how participants feel about AI to begin with. 



% \subsection{Notes}

% 1) safety and risks and 2) privacy - what does the emphasis on this say about a) design recommendations and b) approach to designing/PD of such systems?


% W9 was presented with "Strengths" and "SFBT" output options. They commented, "solution focus is always building on the person's strengths". W9 therefore requested being able to output strengths and SFBT at the same time. But this would suggest that the SFBT output does not currently emphasise strengths strongly enough. However, W9 did not specifically evaluate that, and only made this comment because they saw the "strengths" option available, and in their head, strengths are key to SFBT.
% What does this say about system design and UI in relation to user mental models?

==> sections-old/8_conclusion.tex <==
\section{Conclusion}

In this study, we conducted a series of on-the-ground workshops and focus group discussions to understand the use of generative AI in the social sector. We find that social service practitioners are generally welcoming to AI, and discover that it can potentially be used not just for mundane administrative tasks but also in a range of collaborative discussion scenarios. We elucidate how such systems can be effectively designed through our proposed ACE framework (Attitudes, Considerations, Ethos). We discuss our findings in the context of HAI collaboration and suggest an alternative framing of AI as a (meta-)facilitator - a role that creates and then facilitates new work processes and systems. We then propose key considerations for future system designers, both in social service and beyond, to best harness the potential of generative AI.

==> sections-old/drafts.tex <==
// RELATED WORK

% beyond the small handful of prior work on AI in mental health and ADS risk-assessment systems. While AI tools have quickly become widely adopted in many industries, they can be considered a relative novelty in social work, where AI has begun to gain traction albeit at a sluggish pace \cite{lehtiniemi_contextual_2023, molala_social_2023}. Due to the nascence of AI technologies and the social work sector’s lag in adopting such systems, there is thus a latent gap in the field of applied AI in social work practices \cite{wykman_artificial_2023}, precipitating a need for further exploration. 

% Discuss broadly the background of AI in social work. Machine-assisted decision making can be a subset of this.

% Digital systems that aid social work decision-making generally take the form of predictive risk modelling (PRMs). These are statistical models that predict risks of various outcomes, most notably child abuse or welfare (e.g. \cite{gillingham2019can, van2017predicting}). There is much discussion over the risks involved with using such tools \cite{oak2016minority, drake2020practical}. In a field where decisions are not merely a product of emprical factors \cite{oak2016minority}, decision-aid tools oversimplify cases \cite{fitzgibbon2007risk, broadhurst2010risk} , fail to accurately weigh qualitative factors \cite{shlonsky2005next}, and create ethical dilemmas when tool and worker differ in judgement \cite{dare2012vulnerable}. Their use may also erode practitioners' critical thinking and professional judgement skills \cite{littlechild2008child} and relational competencies in interacting with clients \cite{oak2016minority}. 

% Further, present AI systems often rely on generic models \cite{fitzpatrick2017delivering} and data \cite{gillingham2019can, van2017predicting} that omit specific cultural and individual needs, such as societal norms, localized stigmas, and the unique resources available within one’s social network \cite{rooney2017direct, zhang2021designing}. These factors are crucial to a complete and holistic understanding of a client; existing tools are therefore unable to fully meet the needs of social workers, in providing adequately precise and accurate judgements about their clients.

% The emergence of new AI technologies such as LLMs perpetuate and even exacerbate these problems. By providing more human-like outputs and explanations, they may create a false sense of knowledge and correctness \textit{[cite CASA/related stuff here]}. The new widespread accessibility of such technologies compels a thorough investigation into how they affect the social work profession. At the same time, the opportunities afforded by such technological advancements warrants their use, and therefore an understanding of how they may be implemented responsibly and sustainably.

% The presentation of a singular number can give a sense of false confidence in users. Simply knowing that there is a high statistical risk of something happening to a client does not help them make a clearer judgement. 

% \subsection{AI Assistant Tools?}

% Process-oriented design?

% Why are there some things we did not catch in multiple earlier rounds of PD?

% \subsection{Understanding Use of AI in the Social Sector}
% \label{sec:relatedunderstanding}

% Despite the immense potential of AI systems to augment social work practice, past work has found multiple challenges with integrating such systems into real-life practice. Numerous studies have investigated the use of PRMs to help practitioners decide on a course of action for their clients. Practitioners often experience tension trying to weigh the system's suggestions against their own judgement \cite{kawakami2022improving, saxena2021framework}, being uncertain of how far they should rely on the machine. Despite often being instructed to use the tool as part of evaluating a client, practitioners remain reluctant to fully embrace AI due to its inability to adequately account for the full context of a case \cite{kawakami2022improving, gambrill2001need}, as well as practitioner uncertainty of how the system functioned and what its limitations were \cite{kawakami2022improving}. Brown et al. \cite{brown2019toward} conducted workshops with hypothetical algorithmic tools to understand service providers' comfort levels with using such tools in their work, and found similar issues with mistrust and perceived unreliability. In one instance, the introduction of AI even created new problems of its own, causing contention between confused participants over the inner workings of the tool and how much it should be trusted \cite{kawakami2022improving}. Such factors are critical barriers to the acceptance and effective use of AI in the sector.

% Other studies find a more positive outlook. De-Arteaga et al. \cite{de2020case} investigated how workers responded to a technical glitch resulting in incorrect AI outputs. They found workers "able to appropriately override the tool in many such cases" and make appropriate judgements of their own accord. They reference the spectrum of algorithm aversion and algorithm bias \cite{jones2023people}, finding workers in their study to fall somewhere in the middle of the spectrum.

% \subsection{Understanding Use of AI in Healthcare}
% \label{sec:relatedhealthcare}

% The healthcare sector shares crucial similarities to the social work sector, particularly that 1) practitioners need to make critical decisions that significantly impact a patient's or client's well-being and 2) that practitioners rely on their expert training, judgement, and experience to make the best decision. In healthcare, Decision Support Tools (DST) and their effectiveness in the field are commonly researched in HCI. Past work suggests that many DSTs, once implemented, are rarely used by practitioners, due to a range of factors: a lack of practitioner confidence in system accuracy and disruptions to regular workflows \cite{elwyn2013many}, and lack of agreement with and negative attitudes towards the system \cite{devaraj2014barriers}. Yang et al. \cite{yang2019unremarkable} suggest these challenges can be overcome with the notion of "fairly unremarkable" design: a system that can "be easily passed over when it agrees with [the clinician's] current decision", and "naturally augment the current activities of decision making, rather than pulling clinicians away from doing their routine."

% Many of the issues impeding adoption of clinical DSTs also exist with social work PRMs, specifically that practitioners are unsure of whether, when, and where they should adopt AI recommendations into their work. With the changing landscape of accessible and ubiquitous AI technologies, we re-visit these questions to better understand the challenges and opportunities of modern AI use.

% Find similar applications to ours, but in healthcare
% AI diagnosis - trusted by doctors and patients

% The most commonly-studied tool is the Allegheny Family Screening Tool (AFST) \cite{vaithianathan2017developing}. This outputs a numerical score indicating risk of child rehoming given some parameters input by a human worker. 
% In \citeauthor{kawakami2022improving} study, while workers were expected to use this score as part of their final evaluation of the client, value misalignments and the limitations of the tool's contextual understanding caused workers to rely little on the given score, and instead seek to adjust it according to other factors of the case that the tool does not account for. Further complicating matters, "it was unclear to workers how exactly they were expected to take the AFST’s assessments of long-term risk into account in ways that complemented their own judgment." The inner workings of the tool also became a point of contention. Workers, with their lack of knowledge of the inner workings of the AFST, ended up frequently discussing how the tool arrived at certain judgements, "improvising ways to learn more about the tool themselves". The introduction of this system created a new level of meta-discussion, causing confusion counter-productive to the actual work of assessing and helping clients. Studying the same tool, De-Arteaga et al. \cite{de2020case} investigated how workers responded to a technical glitch in the system, resulting in a subset of its outputs being incorrect. They present a more positive outlook, finding workers "able to appropriately override the tool in many such cases" and make appropriate judgements of their own accord. They reference the spectrum of algorithm aversion and algorithm bias \cite{jones2023people}, finding workers in their study to fall somewhere in the middle of the spectrum. Similar issues plagued other efforts to integrate predictive analytic into child welfare systems \cite{brown2019toward}, with perceptions of unreliable predictions and the uncertainty of how the tool functioned resulting in the termination of two active analytics programs. Brown et al. \cite{brown2019toward} took a different route with hypothetical algorithmic tools and conducted workshops to understand service providers' comfort levels with using such tools in their work. They found data bias and the inability of computers to understand human context to be some of the major factors behind discomfort towards such tools. 

// RESULTS

which are broadly summarized across three high-level thematic categories, which each consist of 3–4 subthemes respectively. \textit{Values} represent the underlying core principles and values that social workers hold in relation to AI use in the social work profession, \textit{Requirements} reflect the explicit translation and manifestation of these principles in concrete design terms and real-world applications of AI, and \textit{Attitudes} are the culmination of the sentiments, thoughts and feelings of social workers that are important for system designers to keep in mind while designing for the acceptance of such systems.

be managed with discretion and nuance. Respect for the client entails providing high quality care to the best ability of the social work practitioner, keeping in mind their individuality and independence while respecting their right to privacy and confidentiality.

While formulating a clear view of a client's situation from these notes is imperative for effective interventions, cleaning up such overwhelming amounts of raw data and formulating them into assessments this process can be difficult and "time-consuming" (W3). This is one area where LLMs and AI, with its superior data processing and generative potential, can "definitely help" with in terms of helping social workers to "streamline [their processes] and save...time" (W1). 

Yet, the use of AI here presents an ethical conundrum. Participants mentioned multiple times how risk and safety concerns (i.e. any potential threats to the physical safety of the client)
Yet, herein lies the ethical conundrum of utilizing AI in social work: it can help social workers to reduce the mental and manual burdens of data cleaning and processing, but before doing so, they need to first and foremost ensure that it is in line with "

These statements show that social workers recognize and value the tremendous time-saving benefits that AI can offer, but are hesitant and cautious about using them due to potential privacy concerns (e.g., whether the AI tool would retain clients' information, or whether the data would be used to train the AI model). , and with the technological advancements and accelerated data processing powers brought about by big data and AI technologies, "[t]oday's social workers face issues involving values and ethics that their predecessors in the profession could not possibly have imagined", including concerns of monitoring, surveillance, data privacy and confidentiality \cite{reamer2018social}. Our interviews therefore underscore the importance of data privacy as a core value of social workers and the exigency of designing and developing ethical AI systems that can safeguard and protect the confidentiality and personal information of clients in the context of social work.

C1's choice of intervention modality "really depends on, like, the case". S6's preparation for a session "depends on what is the goal I want to actually work on with the clients".

This illustrates how different workers may have very different processes and workflows for approaching the same problem (in this case, crafting an intervention plan for a client). Ultimately, however, it is the worker's skills and understanding of how to conceptualize a case using multi-faceted approaches that results in personalized, high-quality care.
This highlights a core \textit{theoretical} competency of social workers and principle behind the profession. Similar to how practitioners respect the individuality of each client \cite{rooney2017direct}, the ability to craft an approach to understanding a client's plight and situation that best fits their situation is a skill that must be accounted for.

\subsubsection{Pedagogy: Training and Learning}

The final theme relates to the ongoing development and growth of social workers, in line with the principle of always seeking to provide the best care possible \cite{rooney2017direct}. Naturally, workers newer to the field do not have all the skills, knowledge, and experience needed to perform parts of their job optimally. W7 had "never attend[ed] CBT training". \textit{[Cite more here...]} As a result, supervision was a theme that came up regularly.

S4 talked about "learning and development"

Proficiency - junior workers lack some skills. Link this to control?

W7 had "never attend[ed] CBT training", and was curious 

While formulating a clear view of a client's situation from these notes is imperative for effective interventions, cleaning up such overwhelming amounts of raw data and formulating them into assessments this process can be difficult and "time-consuming" (W3). This is one area where LLMs and AI, with its superior data processing and generative potential, can "definitely help" with in terms of helping social workers to "streamline [their processes] and save...time" (W1). 

// RESULTS: ATTITUDES

% Across the board, participants expressed surprisingly positive sentiments towards AI, reflecting \textbf{attitudes of openness, amazement and acceptance towards embracing algorithmic technologies in the social service sector}. Most of their interactions with the AI tool and comments revealed a \textit{sense of openness, curiosity, and willingness to experiment with AI}. D1, the director of the center noted that he was "excited [about] this particular project", due to the potential benefits it could bring to the agency and sector. While they acknowledged and were aware of the various limitations and shortcomings of AI, they nonetheless were open towards how they could incorporate it into their existing work practices, and even provide feedback to iteratively test and improve the model. This "willingness to try" spirit was mirrored throughout the testings and FGD with other participants, who were similarly displayed an open-mindedness in their testing the AI tool, gamely trialling the new technology and how they could incorporate it into their existing work practices. The final question in the above quote by D1, "If it's here to stay, how can we make the best of it?" is quite telling of the SSPs' attitude, aptly summarising and reflecting the way participants felt about AI in general: acknowledging the inevitability of AI without rejection or resignation, but rather, with a sense of optimism, acceptance, and positivity in embracing and making the most of it in spite of its challenges. This was similarly paralleled in how other SSPs referred to or talked about AI, stating that "I think there's no harm to use something that makes your life easier" (W5) or that "There's really no harm in terms, it expands the worker's perspective" (S4), viewing AI as a constructive technology that could bring about positive benefits like enhancing their workflows and even helping to broaden their perspectives to thinking and approaching their cases in a new light.

// DISCUSSION

% Human-AI collaboration emerged as a salient theme in the context of digital systems being unable to fully replace human workers in social service. The tendency of GAI to produce information in quantity over quality complements the focused and precise nature of the work normally produced by human workers. Generating multiple possible interventions gave workers new ideas for helping their clients (W11, W12); producing comprehensive overviews of cases helped remind participants of points they might have missed (S5) or expanded their existing perspectives beyond what they might have usually considered (S4); quickly generating summaries and questions about a case provided talking points for supervisors to expand on with junior workers (C1).

% We find this final theme particularly noteworthy because it emphasises the collaborative nature of human-AI interactions, as well as the importance of open dialogue between system designers and users. In our FGDs, we frequently encouraged participants to identify areas in which our system was lacking, even as we also asked them to envision using it in their daily lives. We believe this step to be crucial as it frames participants as the experts, and creates a sense of openness in allowing our users to imagine their own use cases rather than us dictating system design from the perspective of computer scientists.

% \textbf{Where do our findings differ from past work?}

% Going into the sessions, we were uncertain of how our system could help in this regard, since supervision largely involves human-to-human discussion. However, it 

% They conclude by recommending designing tools that "support workers in understanding the boundaries of [an AI system's] capabilities", and implementing design procedures that "support open cultures for critical discussion around AI decision making". The authors outline critical challenges of implementing AI systems, elucidating factors that may hinder their effectiveness and even negatively affect operations within the organisation.

% \subsection{explain possible reasons for results}
% May not be relevant to our paper

==> sections/0_abstract.tex <==
\begin{abstract}
In social service, administrative burdens and decision-making challenges often hinder practitioners from performing effective casework. Generative AI (GenAI) offers significant potential to streamline these tasks, yet exacerbates concerns about overreliance, algorithmic bias, and loss of identity within the profession. We explore these issues through a two-stage participatory design study. We conducted formative co-design workshops (\textit{n=27}) to create a prototype GenAI tool, followed by contextual inquiry sessions with practitioners (\textit{n=24}) using the tool with real case data. We reveal opportunities for AI integration in documentation, assessment, and worker supervision, while highlighting risks related to GenAI limitations, skill retention, and client safety. Drawing comparisons with GenAI tools in other fields, we discuss design and usage guidelines for such tools in social service practice.
\end{abstract}

==> sections/drafts.tex <==
// RELATED WORK

% beyond the small handful of prior work on AI in mental health and ADS risk-assessment systems. While AI tools have quickly become widely adopted in many industries, they can be considered a relative novelty in social work, where AI has begun to gain traction albeit at a sluggish pace \cite{lehtiniemi_contextual_2023, molala_social_2023}. Due to the nascence of AI technologies and the social work sector’s lag in adopting such systems, there is thus a latent gap in the field of applied AI in social work practices \cite{wykman_artificial_2023}, precipitating a need for further exploration. 

% Discuss broadly the background of AI in social work. Machine-assisted decision making can be a subset of this.

% Digital systems that aid social work decision-making generally take the form of predictive risk modelling (PRMs). These are statistical models that predict risks of various outcomes, most notably child abuse or welfare (e.g. \cite{gillingham2019can, van2017predicting}). There is much discussion over the risks involved with using such tools \cite{oak2016minority, drake2020practical}. In a field where decisions are not merely a product of emprical factors \cite{oak2016minority}, decision-aid tools oversimplify cases \cite{fitzgibbon2007risk, broadhurst2010risk} , fail to accurately weigh qualitative factors \cite{shlonsky2005next}, and create ethical dilemmas when tool and worker differ in judgement \cite{dare2012vulnerable}. Their use may also erode practitioners' critical thinking and professional judgement skills \cite{littlechild2008child} and relational competencies in interacting with clients \cite{oak2016minority}. 

% Further, present AI systems often rely on generic models \cite{fitzpatrick2017delivering} and data \cite{gillingham2019can, van2017predicting} that omit specific cultural and individual needs, such as societal norms, localized stigmas, and the unique resources available within one’s social network \cite{rooney2017direct, zhang2021designing}. These factors are crucial to a complete and holistic understanding of a client; existing tools are therefore unable to fully meet the needs of social workers, in providing adequately precise and accurate judgements about their clients.

% The emergence of new AI technologies such as LLMs perpetuate and even exacerbate these problems. By providing more human-like outputs and explanations, they may create a false sense of knowledge and correctness \textit{[cite CASA/related stuff here]}. The new widespread accessibility of such technologies compels a thorough investigation into how they affect the social work profession. At the same time, the opportunities afforded by such technological advancements warrants their use, and therefore an understanding of how they may be implemented responsibly and sustainably.

% The presentation of a singular number can give a sense of false confidence in users. Simply knowing that there is a high statistical risk of something happening to a client does not help them make a clearer judgement. 

% \subsection{AI Assistant Tools?}

% Process-oriented design?

% Why are there some things we did not catch in multiple earlier rounds of PD?

% \subsection{Understanding Use of AI in the Social Sector}
% \label{sec:relatedunderstanding}

% Despite the immense potential of AI systems to augment social work practice, past work has found multiple challenges with integrating such systems into real-life practice. Numerous studies have investigated the use of PRMs to help practitioners decide on a course of action for their clients. Practitioners often experience tension trying to weigh the system's suggestions against their own judgement \cite{kawakami2022improving, saxena2021framework}, being uncertain of how far they should rely on the machine. Despite often being instructed to use the tool as part of evaluating a client, practitioners remain reluctant to fully embrace AI due to its inability to adequately account for the full context of a case \cite{kawakami2022improving, gambrill2001need}, as well as practitioner uncertainty of how the system functioned and what its limitations were \cite{kawakami2022improving}. Brown et al. \cite{brown2019toward} conducted workshops with hypothetical algorithmic tools to understand service providers' comfort levels with using such tools in their work, and found similar issues with mistrust and perceived unreliability. In one instance, the introduction of AI even created new problems of its own, causing contention between confused participants over the inner workings of the tool and how much it should be trusted \cite{kawakami2022improving}. Such factors are critical barriers to the acceptance and effective use of AI in the sector.

% Other studies find a more positive outlook. De-Arteaga et al. \cite{de2020case} investigated how workers responded to a technical glitch resulting in incorrect AI outputs. They found workers "able to appropriately override the tool in many such cases" and make appropriate judgements of their own accord. They reference the spectrum of algorithm aversion and algorithm bias \cite{jones2023people}, finding workers in their study to fall somewhere in the middle of the spectrum.

% \subsection{Understanding Use of AI in Healthcare}
% \label{sec:relatedhealthcare}

% The healthcare sector shares crucial similarities to the social work sector, particularly that 1) practitioners need to make critical decisions that significantly impact a patient's or client's well-being and 2) that practitioners rely on their expert training, judgement, and experience to make the best decision. In healthcare, Decision Support Tools (DST) and their effectiveness in the field are commonly researched in HCI. Past work suggests that many DSTs, once implemented, are rarely used by practitioners, due to a range of factors: a lack of practitioner confidence in system accuracy and disruptions to regular workflows \cite{elwyn2013many}, and lack of agreement with and negative attitudes towards the system \cite{devaraj2014barriers}. Yang et al. \cite{yang2019unremarkable} suggest these challenges can be overcome with the notion of "fairly unremarkable" design: a system that can "be easily passed over when it agrees with [the clinician's] current decision", and "naturally augment the current activities of decision making, rather than pulling clinicians away from doing their routine."

% Many of the issues impeding adoption of clinical DSTs also exist with social work PRMs, specifically that practitioners are unsure of whether, when, and where they should adopt AI recommendations into their work. With the changing landscape of accessible and ubiquitous AI technologies, we re-visit these questions to better understand the challenges and opportunities of modern AI use.

% Find similar applications to ours, but in healthcare
% AI diagnosis - trusted by doctors and patients

% The most commonly-studied tool is the Allegheny Family Screening Tool (AFST) \cite{vaithianathan2017developing}. This outputs a numerical score indicating risk of child rehoming given some parameters input by a human worker. 
% In \citeauthor{kawakami2022improving} study, while workers were expected to use this score as part of their final evaluation of the client, value misalignments and the limitations of the tool's contextual understanding caused workers to rely little on the given score, and instead seek to adjust it according to other factors of the case that the tool does not account for. Further complicating matters, "it was unclear to workers how exactly they were expected to take the AFST’s assessments of long-term risk into account in ways that complemented their own judgment." The inner workings of the tool also became a point of contention. Workers, with their lack of knowledge of the inner workings of the AFST, ended up frequently discussing how the tool arrived at certain judgements, "improvising ways to learn more about the tool themselves". The introduction of this system created a new level of meta-discussion, causing confusion counter-productive to the actual work of assessing and helping clients. Studying the same tool, De-Arteaga et al. \cite{de2020case} investigated how workers responded to a technical glitch in the system, resulting in a subset of its outputs being incorrect. They present a more positive outlook, finding workers "able to appropriately override the tool in many such cases" and make appropriate judgements of their own accord. They reference the spectrum of algorithm aversion and algorithm bias \cite{jones2023people}, finding workers in their study to fall somewhere in the middle of the spectrum. Similar issues plagued other efforts to integrate predictive analytic into child welfare systems \cite{brown2019toward}, with perceptions of unreliable predictions and the uncertainty of how the tool functioned resulting in the termination of two active analytics programs. Brown et al. \cite{brown2019toward} took a different route with hypothetical algorithmic tools and conducted workshops to understand service providers' comfort levels with using such tools in their work. They found data bias and the inability of computers to understand human context to be some of the major factors behind discomfort towards such tools. 

// RESULTS

which are broadly summarized across three high-level thematic categories, which each consist of 3–4 subthemes respectively. \textit{Values} represent the underlying core principles and values that social workers hold in relation to AI use in the social work profession, \textit{Requirements} reflect the explicit translation and manifestation of these principles in concrete design terms and real-world applications of AI, and \textit{Attitudes} are the culmination of the sentiments, thoughts and feelings of social workers that are important for system designers to keep in mind while designing for the acceptance of such systems.

be managed with discretion and nuance. Respect for the client entails providing high quality care to the best ability of the social work practitioner, keeping in mind their individuality and independence while respecting their right to privacy and confidentiality.

While formulating a clear view of a client's situation from these notes is imperative for effective interventions, cleaning up such overwhelming amounts of raw data and formulating them into assessments this process can be difficult and "time-consuming" (W3). This is one area where LLMs and AI, with its superior data processing and generative potential, can "definitely help" with in terms of helping social workers to "streamline [their processes] and save...time" (W1). 

Yet, the use of AI here presents an ethical conundrum. Participants mentioned multiple times how risk and safety concerns (i.e. any potential threats to the physical safety of the client)
Yet, herein lies the ethical conundrum of utilizing AI in social work: it can help social workers to reduce the mental and manual burdens of data cleaning and processing, but before doing so, they need to first and foremost ensure that it is in line with "

These statements show that social workers recognize and value the tremendous time-saving benefits that AI can offer, but are hesitant and cautious about using them due to potential privacy concerns (e.g., whether the AI tool would retain clients' information, or whether the data would be used to train the AI model). , and with the technological advancements and accelerated data processing powers brought about by big data and AI technologies, "[t]oday's social workers face issues involving values and ethics that their predecessors in the profession could not possibly have imagined", including concerns of monitoring, surveillance, data privacy and confidentiality \cite{reamer2018social}. Our interviews therefore underscore the importance of data privacy as a core value of social workers and the exigency of designing and developing ethical AI systems that can safeguard and protect the confidentiality and personal information of clients in the context of social work.

C1's choice of intervention modality "really depends on, like, the case". S6's preparation for a session "depends on what is the goal I want to actually work on with the clients".

This illustrates how different workers may have very different processes and workflows for approaching the same problem (in this case, crafting an intervention plan for a client). Ultimately, however, it is the worker's skills and understanding of how to conceptualize a case using multi-faceted approaches that results in personalized, high-quality care.
This highlights a core \textit{theoretical} competency of social workers and principle behind the profession. Similar to how practitioners respect the individuality of each client \cite{rooney2017direct}, the ability to craft an approach to understanding a client's plight and situation that best fits their situation is a skill that must be accounted for.

\subsubsection{Pedagogy: Training and Learning}

The final theme relates to the ongoing development and growth of social workers, in line with the principle of always seeking to provide the best care possible \cite{rooney2017direct}. Naturally, workers newer to the field do not have all the skills, knowledge, and experience needed to perform parts of their job optimally. W7 had "never attend[ed] CBT training". \textit{[Cite more here...]} As a result, supervision was a theme that came up regularly.

S4 talked about "learning and development"

Proficiency - junior workers lack some skills. Link this to control?

W7 had "never attend[ed] CBT training", and was curious 

While formulating a clear view of a client's situation from these notes is imperative for effective interventions, cleaning up such overwhelming amounts of raw data and formulating them into assessments this process can be difficult and "time-consuming" (W3). This is one area where LLMs and AI, with its superior data processing and generative potential, can "definitely help" with in terms of helping social workers to "streamline [their processes] and save...time" (W1). 

// RESULTS: ATTITUDES

% Across the board, participants expressed surprisingly positive sentiments towards AI, reflecting \textbf{attitudes of openness, amazement and acceptance towards embracing algorithmic technologies in the social service sector}. Most of their interactions with the AI tool and comments revealed a \textit{sense of openness, curiosity, and willingness to experiment with AI}. D1, the director of the center noted that he was "excited [about] this particular project", due to the potential benefits it could bring to the agency and sector. While they acknowledged and were aware of the various limitations and shortcomings of AI, they nonetheless were open towards how they could incorporate it into their existing work practices, and even provide feedback to iteratively test and improve the model. This "willingness to try" spirit was mirrored throughout the testings and FGD with other participants, who were similarly displayed an open-mindedness in their testing the AI tool, gamely trialling the new technology and how they could incorporate it into their existing work practices. The final question in the above quote by D1, "If it's here to stay, how can we make the best of it?" is quite telling of the SSPs' attitude, aptly summarising and reflecting the way participants felt about AI in general: acknowledging the inevitability of AI without rejection or resignation, but rather, with a sense of optimism, acceptance, and positivity in embracing and making the most of it in spite of its challenges. This was similarly paralleled in how other SSPs referred to or talked about AI, stating that "I think there's no harm to use something that makes your life easier" (W5) or that "There's really no harm in terms, it expands the worker's perspective" (S4), viewing AI as a constructive technology that could bring about positive benefits like enhancing their workflows and even helping to broaden their perspectives to thinking and approaching their cases in a new light.

// DISCUSSION

% Human-AI collaboration emerged as a salient theme in the context of digital systems being unable to fully replace human workers in social service. The tendency of GAI to produce information in quantity over quality complements the focused and precise nature of the work normally produced by human workers. Generating multiple possible interventions gave workers new ideas for helping their clients (W11, W12); producing comprehensive overviews of cases helped remind participants of points they might have missed (S5) or expanded their existing perspectives beyond what they might have usually considered (S4); quickly generating summaries and questions about a case provided talking points for supervisors to expand on with junior workers (C1).

% We find this final theme particularly noteworthy because it emphasises the collaborative nature of human-AI interactions, as well as the importance of open dialogue between system designers and users. In our FGDs, we frequently encouraged participants to identify areas in which our system was lacking, even as we also asked them to envision using it in their daily lives. We believe this step to be crucial as it frames participants as the experts, and creates a sense of openness in allowing our users to imagine their own use cases rather than us dictating system design from the perspective of computer scientists.

% \textbf{Where do our findings differ from past work?}

% Going into the sessions, we were uncertain of how our system could help in this regard, since supervision largely involves human-to-human discussion. However, it 

% They conclude by recommending designing tools that "support workers in understanding the boundaries of [an AI system's] capabilities", and implementing design procedures that "support open cultures for critical discussion around AI decision making". The authors outline critical challenges of implementing AI systems, elucidating factors that may hinder their effectiveness and even negatively affect operations within the organisation.

% \subsection{explain possible reasons for results}
% May not be relevant to our paper
